Time-Robust Path Planning with Piece-Wise Linear Trajectory for Signal Temporal Logic Specifications

Real-world scenarios are characterized by timing uncertainties, e.g., delays, and disturbances. Algorithms with temporal robustness are crucial in guaranteeing the successful execution of tasks and missions in such scenarios. We study time-robust path planning for synthesizing robots' trajectories that adhere to spatial-temporal specifications expressed in Signal Temporal Logic (STL). In contrast to prior approaches that rely on {discretize}d trajectories with fixed time steps, we leverage Piece-Wise Linear (PWL) signals for the synthesis. PWL signals represent a trajectory through a sequence of time-stamped waypoints. This allows us to encode the STL formula into a Mixed-Integer Linear Program (MILP) with fewer variables. This reduction is more pronounced for specifications with a long planning horizon. To that end, we define time-robustness for PWL signals. Subsequently, we propose quantitative semantics for PWL signals according to the recursive syntax of STL and prove their soundness. We then propose an encoding strategy to transform our semantics into a MILP. Our simulations showcase the soundness and the performance of our algorithm.

==> sections/apx_algo.tex <==
\section{Time-Robust STL Synthesis} \label{apx:algo2}
\begin{algorithm}[H] 
\caption{Time-Robust Synthesis with MILP}
\label{alg:all_in}
\begin{algorithmic}[1]
\Require{STL Formula $\lgSpec$, number of waypoints $K$, maximal velocity $v_b > 0$, makespan $T > 0$} 
\Ensure{${\xi_{z_0}}$}
    \Statex{// Setup}
    \State Initialize decision variables ${\xi_{z_0}}$
    \State \cstrSetFinal $\gets$ \{\}
    
    \Statex{// STL constraints}
    \For{ each region $\mathcal{P}$ in $\lgSpec$}   
    \State \cstrSet $\gets$ Algorithm \ref{alg:sr_ra}($\mathcal{P}$, $\lgSpec$, $K$, $\xi_{z_0}$) 
    \State \cstrSetFinal $\gets$ \{\cstrSetFinal, \cstrSet\}
    \EndFor

    \Statex{// Dynamic constraints for the waypoints}
    \State \cstrSetFinal $\gets$ \{\cstrSetFinal, $t_0 = 0, t_{K-1} = T$\}
    \Statex    
    {// Loop over each pair of waypoints $\tuple{t_i, p_i, t_{i+1}, p_{i+1}}$}
    \For{i $\gets$ 0 to $K-1$}   
    \State \cstrSetFinal $\gets$ \{\cstrSetFinal, $t_{i+1} \geq t_{i}, |p_{i+1} - p_{i}| \leq v_b (t_{i+1} - t_{i})$\}
    \EndFor

    \State{// MILP Synthesis}
    \State ${\xi_{z_0}}$ $\gets$ GUROBI(\cstrSetFinal, $J({\xi_{z_0}})$)    
\end{algorithmic}
\end{algorithm}

==> sections/apx_enc_milp.tex <==

Similarly for the "always" operator, recall the definition from \eqref{eq:alws_time_rob_strict} and let $\trob^*$ be $\trobzj{i}^{\stlAlways{a,b}\lgSpec}$, we impose the following constraints
\begin{flalign*}    
&\trobzj{j}^\lgSpec - (1- b_{j})M \leq \trob^* \leq \trobzj{j}^\lgSpec + (1- b_{ij}^\intersect)M, ~ \forall j \in \{1 \cdots K\},\\ 
& b_{ij}^\intersect = [t_j, t_{j+1}] \intersect [t_{i} +a, t_{i+1} + b] \neq \varnothing, b_{ij}^\intersect \geq b_j, \sum_{j = 1}^K b_j = 1. 
\end{flalign*}
\thought{
\begin{remark}
Did we introduce any conservatism here?
\end{remark}
}
The encoding for the "until" operator is performed similarly. 
% \begin{align*}
%     \trob^{\phi_1\stlUntil{a,b}\phi_2}(z_i) &= \max_{j \in \set{J}^\intersect}\left( \min \left( \trob^{\phi_2}(z_j), \min_{l \in \set{L}_j^\intersect}\trob^{\phi_1}(z_l) \right)\right), \\
% \set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \set{L}^\intersect_j = \left\{1 \cdots j | b^\intersect_{il} = 1\right\}, \\
% b^\intersect_{ij} &= ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing, \\
% b^\intersect_{il} &= [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing.
% \end{align*}
Let $\trobzj{i}^*$ be the time-robustness of the until operator that we want to derive. To encode the inner $\min$ operator, we denote them as $K$ continuous variables
\begin{align*}    
&[\underline{\trobzj{1}}, \cdots, \underline{\trobzj{K}}] = [{\min_{l \in \set{L}_1^\intersect}(\trobzj{1}^{\phi_2}, \trobzj{l}^{\phi_1}}), \cdots ,{\min_{l \in \set{L}_K^\intersect}(\trobzj{K}^{\phi_2}, \trobzj{l}^{\phi_1}})], 
\end{align*}
where ${\set{L}^\intersect_j = \left\{1 \cdots j | b^\intersect_{il} = ([t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing) =  1\right\}}$. Recall that the time intersection set of the outer $\max$ operator is defined as ${\set{J}^\intersect = \left\{1 \cdots K | b^\intersect_{ij} = ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing) 
 = 1\right\}}$, we rewrite the time robustness of the "until" operator as follows.
\begin{flalign*}
& \forall j \in \{1 \cdots K\}, b^\intersect_{ij} = 1 \hequal \forall j \in \set{J}^\intersect \implies \trobzj{i}^* \geq \underline{\trobzj{j}}, \\
& \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2} \lgAnd \left(\forall l \in \{1 \cdots j\}, b^\intersect_{il} = 1 \hequal \forall l \in \set{L}^\intersect_j \implies (\underline{\trobzj{j}} \leq \trobzj{l}^{\lgSpec_1})\right).
\end{flalign*}
For each $\underline{\trobzj{j}} = \min_{l \in \set{L}_j^\intersect (\trobzj{j}^{\phi_2}, \trobzj{l}^{\phi_1}})$, we use $j+1$ additional binary variables $[\bmin{1}^j, \bmin{2}^j, \cdots, \bmin{j}^j, \bmin{j+1}^j]$ with $\sum_{l = 1}^{j+1} \bmin{l}^j = 1$ and impose the following constraints
\begin{nalign}
& \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2}, \trobzj{j}^{\lgSpec_2} - (1- \bmin{j+1}^j)M \leq \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2} + (1- \bmin{j+1}^j)M,\\ 
& \forall l \in \{1 \cdots j\}, b_{il}^\intersect \geq \bmin{l}^j, \trobzj{l}^{\lgSpec_1} - (1- \bmin{l}^j)M \leq \underline{\trobzj{j}} \leq \trobzj{l}^{\lgSpec_1} + (1- b_{il}^\intersect)M.\\
\end{nalign}
Afterwards, we encode the outer $\max$ operators considering time intersection, we introduce $K$ additional binary variables $[\bmax{1}, \bmax{2} \cdots \bmax{K}]$ with $\sum_{j = 1}^K \bmax{j} = 1$ and impose the following constraints for all $j \in \{1 \cdots K\}$
\begin{flalign*}
& \underline{\trobzj{j}} - (1- b^\intersect_{ij})M \leq \trobzj{i}^* \leq \underline{\trobzj{j}} + (1- \bmax{j})M, ~b^\intersect_{ij} \geq \bmax{j}. 
\end{flalign*}

\begin{remark}
    We use $\bigO(K^2)$ binary variables and $\bigO(K)$ continuous variables to encode the "until" operators. \thought{The encoding is sound, but I will double-check it later if we can further reduce the complexity.}
\end{remark}


==> sections/apx_exp_hw.tex <==
\section{Hardware and Implementation Information} \label{apx:hw_info}
The experiments are performed on a Lenovo ThinkCentre M75-q2-gen2 computer with AMD Ryzen 7 4750GE, 3.1 Ghz, 16 Gb RAM, and running Linux OS. We use YALMIP \footnote{YALMIP - "https://yalmip.github.io/"} and MATLAB \footnote{MATLAB 2022b - "https://www.mathworks.com"} to implement the \ac{MILP} encoding. The optimization solver is Gurobi \footnote{Gurobi 10.0.1 - "https://www.gurobi.com"}.


==> sections/apx_mod_tr.tex <==
\section{Proof of Theorem \ref{theorem:soundness}} \label{apd:mod_tr}
We show the following property holds
\begin{nalign}
    \trob^{\phi}(z_i) &> 0 \implies z_i^\phi = ~\lgTrue \hequal (\xi, t_i) \lgSatisfy \phi \\ 
    %\trob^{\phi}(z_i) &< 0 \implies z_i^\phi = ~\lgFalse \hequal (\xi, t_i) \not \lgSatisfy \phi
\end{nalign}

\begin{proof}
The proof is derived recursively according to induction hypothesis, i.e., the soundness of a formula is derived from the soundness of its sub-formulas.

\begin{enumerate}[leftmargin=*]
\item Proposition $\pi$:
\begin{align*}
    \theta_{+,z_i}^{\pi} &= \sign(z_i) \sum_{j = i}^{i + k}(t_{j+1} - t_j), \\ 
    k &= \argmax_{\{0, 1, \cdots, K\}} \forall i^\prime \in \{i+1, \cdots, i+k\}, \sign(z_i) = \sign(z_{i^\prime});
    % \theta_{-,z_i}^{\pi} &= \sign(z_i) \sum_{j = i-k}^{i}(t_{j+1} - t_j), \\
    % k &= \argmax_{\{0, 1, \cdots, K\}} \forall i^\prime \in \{i-k, \cdots, i-1\}, \sign(z_i) = \sign(z_{i^\prime}).
\end{align*}

% $\trobr^\lgSpec(z_i) > 0 \implies z_i^\phi = \lgTrue:$
\begin{flalign*}
    & \rtrobzj{i}^\pi > 0 \implies  \sign(z_i)\sum_{j = i}^{i + k}(t_{j+1} - t_j) > 0. &&\\
    &\text{Since }(t_{j+1} - t_j) \geq 0 ~\forall j \text{~and~} \sign(z_j) = \sign(z_i) \neq 0,&& \\
    &\sign(z_i)\sum_{j = i}^{i + k}(t_{j+1} - t_j) > 0 \implies \sign(z_i)= 1 &&\\
    & \iff  z_i^\pi = \lgTrue \iff (\xi, t_i) \lgSatisfy \pi.&&
\end{flalign*}

\item Negation $\lgNeg \pi$: \\
A similar derivation is applied for the negation, we have
\begin{flalign*}
   \trobr^{\tlNot\pi}(z_i) < 0 \implies \sign(z_i) < 0 \iff z_i \lgSatisfy \tlNot\pi \text{~or~} z_i \not\lgSatisfy \pi. &&
\end{flalign*}

\item Conjunction $\lgSpec_1 \lgAnd \lgSpec_2: \trobzj{i}^{\lgSpec_1 \lgAnd \lgSpec_2} = \min \left( \trobzj{i}^{\lgSpec_1}, \trobzj{i}^{\lgSpec_2}\right)$:
\begin{flalign*}
    & \trobzj{i}^{\lgSpec_1 \lgAnd \lgSpec_2} > 0 \implies (\trobzj{i}^{\lgSpec_1} > 0 \lgAnd \trobzj{i}^{\lgSpec_2} > 0). &&
\end{flalign*}
From induction hypothesis, we have
\begin{flalign*}
 & \trobzj{i}^{\lgSpec_1} > 0 \lgAnd \trobzj{i}^{\lgSpec_2} > 0 \implies z_i^{\lgSpec_1} = \lgTrue \lgAnd z_i^{\lgSpec_2} = \lgTrue &&\\ 
 & \implies z_i^{\lgSpec_1 \lgAnd \lgSpec_2} = \lgTrue. \end{flalign*}

\item Temporal Operators 
\begin{itemize} [wide, labelwidth=!, labelindent=0pt]
\item Until Operator $\lgSpec_1 \stlUntil{a,b} \lgSpec_2:$

Qualitative Semantics
\begin{flalign*}
%  \trobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \max_{j \in \set{J}^\intersect}\left( \min \left( \trobzj{j}^{\phi_2}, \min_{l \in \set{L}_j^\intersect}\trobzj{l}^{\phi_1} \right)\right), \\
% \set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \set{L}^\intersect_j = \left\{1 \cdots j | b^\intersect_{il} = 1\right\}, \\
% b^\intersect_{ij} &= ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing, \\
% b^\intersect_{il} &= [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing. \\
%
z_{i}^{\lgSpec_1\stlUntil{a,b}\lgSpec_2} &: \exists t^\prime \in [t_{i+1} + a, t_i +b], \\
    & \hspace*{-1cm} \bigvee_{j = 1}^{K} \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec_2} \lgAnd \bigvee_{l = 0}^j \left(t^\prime \in [t_l, t_{l+1}] \implies z_l^{\lgSpec_1}\right)\right)
\end{flalign*}

Quantitative Semantics
\begin{flalign*}
\rtrobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \max_{j \in \set{J}^\intersect}\left( \min \left(\rtrobzj{j}^{\phi_2}, \min_{l \in \set{L}_j^\intersect}\rtrobzj{l}^{\phi_1} + (t_l - (t_i + b)) \right)\right),\\
\ltrobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \max_{j \in \set{J}^\intersect}\left( \min \left(\ltrobzj{j}^{\phi_2}, \min_{l \in \set{L}_j^\intersect}\ltrobzj{l}^{\phi_1} + ((t_i + a) - t_l) \right)\right),\\
\set{J}^\intersect &= \left\{1 \cdots K | t^\prime \in (t_j, t_{j+1}]\right\}, \set{L}^\intersect_j = \left\{1 \cdots j | t^\prime \in [t_l, t_{l+1}]\right\}, \\
% b^\intersect_{ij} &= (, \\
% b^\intersect_{il} &=  \\
t_{i+1} + a &\leq t^\prime \leq t_i +b.
\end{flalign*}

\hrzline{0.5}
\item $\stlEvtll{a,b} \lgSpec = \lgTrue\stlUntil{a,b}\lgSpec$
\begin{nalign} 
z_{i}^{\stlEvtll{a,b}\lgSpec} &= z_{i}^{\lgTrue \stlUntil{a,b}\lgSpec}: \\
&\exists t^\prime \in [t_{i+1} + a, t_i +b], \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec_2} \right) \\
\hequal \bigvee_{j = 1}^{K} &\left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec_2} \right). 
\end{nalign}

\begin{nalign} 
\trobzj{i}^{\stlEvtll{a,b}\lgSpec} &= \trobzj{i}^{\lgTrue \stlUntil{a,b}\lgSpec}: \exists t^\prime \in [t_{i+1} + a, t_i +b]
\end{nalign}

\hrzline{0.5}
\item $\stlAlways{a,b} \lgSpec = \tlNot (\stlEvtll{a,b} \tlNot \lgSpec)$

Time robustness is encoded recursively for the temporal operators according to Definition \ref{def:quanti_tr} as follows:
\begin{flalign*} 
\rtrobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \rtrobzj{j}^\phi + (t_j - (t_{i+1} +b)), \\
\ltrobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \ltrobzj{j}^\phi - (t_{j+1} - (t_{i} +a)), \\
% \trobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \\
\set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \\ 
{b^\intersect_{ij}} &= \left([t_j, t_j+1] \intersect [t_i + a, t_{i+1} + b] \right).
\end{flalign*}
%

\end{itemize}


\end{enumerate}

\end{proof}

\begin{figure}
    \hspace*{-0.5cm}\subfloat[Strict $\theta$
      \label{fig:exp-a}]{\includegraphics[width = 0.27\textwidth]{figs/Test UAV PWL Strict.png}}
    \subfloat[Modified $\theta$
      \label{fig:exp-a}]{\includegraphics[width = 0.285\textwidth]{figs/Test UAV PWL Mod.png}} \par
    \caption{Result of Strict and Modified Time Robustness Encoding for ${\lgSpec = \stlAlways{20,30} (z \geq 20) \lgAnd \stlAlways{60,70} (z \leq 10)}$.}
    \label{fig:strict_vs_modi}
\end{figure} 
























==> sections/backup.tex <==
\subsection{Backup}
We also provide the derivation of "Eventually" and "Always" operators from the "Until" operator.

$\stlEvtll{a,b} \lgSpec \hequal \lgTrue\stlUntil{a,b}\lgSpec$:
\begin{align*} 
z_{i}^{\stlEvtll{a,b}\lgSpec} &= z_{i}^{\lgTrue \stlUntil{a,b}\lgSpec} \\
& \hequal \exists t^\prime \in [t_{i+1} + a, t_i +b], \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec} \right) \\
& \hequal \bigvee_{j = 1}^{K} \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec} \right).  
\end{align*}

\hrzline{0.5}
$\stlAlways{a,b} \lgSpec \hequal \tlNot (\stlEvtll{a,b} \tlNot \lgSpec)$:
\begin{align*} 
z_{i}^{\stlAlways{a,b}\lgSpec} & \hequal \lgNeg \left(\bigvee_{j = 1}^{K} \left(t^\prime \in [t_{i+1} + a, t_i +b] \lgAnd t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgNeg \lgSpec} \right) \right) \\
& \hequal \bigwedge_{j=1}^K \left(t^\prime \in [t_j, t_{j+1}] \lgAnd \lgNeg z_j^{\lgSpec} \right) \hequal \bigwedge_{j=1}^K \left(t^\prime \not \in [t_j, t_{j+1}] \lgOr \lgNeg z_j^{\lgSpec} \right)
\end{align*}


\begin{table*}    
\begin{center}
\caption{BENCHMARK}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| } 
 \hline
 %\multicolumn{7}{|c|}{$\lgSpec = \stlAlways{20,30} (z \geq 20) \lgAnd \stlAlways{60,70} (z \leq 10)$} \\
 %\hline
%\multirow{1}{*}{Type}
 
 \multicolumn{1}{|c|}{} &\multicolumn{2}{|c|}{Trajectory} &\multicolumn{4}{|c|}{MILP Info} & \multicolumn{2}{|c|}{Time [s]} & \\\hline 
 STL & Type & K/T &\# Cstr & \# Bin & \# Cont & Obj & GRB& YM &Notes\\
% HBLT
% \hline
% \multirow{2}{*}{$\lgSpec$} 
% & PWL & K & cstr (-) & bin (-) & cont (-) & obj & grb & ym & Notes \\
% & IB  & T & cstr (-) & bin (-) & cont (-) & obj & grb & ym & notes \\
% % UAV
% \hline
% \multirow{2}{*}{$\lgSpec_1$} 
% & PWL & 23 & 652 & 146 & 95 & $\theta_+$ = 22 & 0.9 & 3.5 &\\
% & IB & 100 & 2447 & 224 & 502 & $\theta_+$ = 23 & 1.5 & 0.58&\\
% MB1
\hline
\multirow{3}{*}{$\lgSpec_1$ MB1} 
& PWL & 23 & 14122 (22740) & 4598 (7724) & 658 (895) & L = 44.72 $\theta$ = 21.8 & 14* & 7.6 & 13\_07\_16\_33\_25 \\
& PWL & 25 & 17504 (25764) & 5722 (8810) & 798 (975) & L = 44.72 $\theta$ = 21.8 & 26-165 & 8.7 & 13\_07\_16\_46\_39 \\
& PWL & 30 & 25733 (34024) & 8966 (11805) & 1012 (1175) & L = 44.72 $\theta$ = 21.8 & 165-x & 8.7 & 13\_07\_18\_20\_25 \\
& IB & 100 & 10292 (29214) & 3792 (7215) & 720 (2959) & L = 44.72 $\theta$ = 23 & 62-95 & 9.3 & 13\_07\_16\_37\_18 \\
% \hline
% \multirow{2}{*}{$\lgSpec_1$ MB1} 
% & PWL & K & cstr (-) & bin (-) & cont (-) & obj & grb & ym & 09\_07\_14\_56\_32 \\
% & DT & T & cstr (-) & bin (-) & cont (-) & obj & grb & ym & notes \\
% MB2
\hline
\multirow{2}{*}{$\lgSpec_2$ MB2} 
& PWL & 25 & 37794 (49581) & 13120 (16636) & 1736 (1973) & L = 80 $\theta$ = 17.73 & 29* & 17 & 16\_07\_14\_00\_29 [0 -1]\\
& PWL & 25 & 33855 (49677) & 11249 (16636) & 1736 (1973) & L = 71.4 $\theta$ = 17.73 & 38* & 17 & 16\_07\_12\_54\_32 [1 -1]\\
& PWL & 27 & 38709 (55371) & 13053 (18646) & 1725 (2187) & L = 70 $\theta$ = 17.73 & 86-160*-195 & 19 & 16\_07\_12\_45\_18 [1 -1]\\
& IB & 300 & 68349 (192532) & 26713 (48275) & 3340 (16487) & L = 70 $\theta$ = 17  & 16-630*-x & 66 & 16\_07\_13\_08\_36 [1 -1] \\ 
& IB & 300 & 69995 (191336) & 28072 (48275) & 2776 (15889) & L = 207.3 $\theta$ = 17 & 65 & 66 & 16\_07\_13\_45\_58 [0 -1] \\ 
% DP1
\hline
\multirow{4}{*}{$\lgSpec_3$ DP1} 
& PWL & 23 & 12476 (18498) & 4098 (6394) & 531 (648) & L = 75 $\theta$ = 0.2 & 6 & ym & 14\_07\_10\_27\_05 \\
& PWL & 25 & 14764 (21209) & 4928 (7383) & 586 (706) & L = 76 $\theta$ = 9.7 & 27 & 7.2 & 14\_07\_10\_29\_24 \\
& PWL & 30 & 21975 (28739) & 7761 (10153) & 758 (851) & L = 76 $\theta$ = 9.7 & 149*-1e3 & 9.9 & 14\_07\_10\_46\_42 \\
& IB & 100 & 13620 (21874) & 2425 (5537) & 1046 (2358) & L = 76 $\theta$ = 10 & 78-6e2 & 7.4 & 15\_07\_13\_22\_20  \\
\hline
% \multirow{2}{*}{DP1-L} 
% & PWL & 27 & cstr (-) & bin (-) & cont (-) & obj & grb & ym & ... \\
% & DT & 200 & cstr (-) & bin (-) & cont (-) & obj & grb & ym & ... \\
% DP 2
%\hline
\multirow{2}{*}{$\lgSpec_4$ DP2} 
& PWL & 35 & 21681 (39337) & 6218 (11855) & 1634 (2090) & L = 152 $\theta$  = 10 & 251-305 & 13.5 & 15\_07\_12\_33\_07 \\
& PWL & 40 & 27619 (46577) & 8105 (14085) & 1950 (2395) & L = 143 $\theta$  = 14.2 & 491-904-x & 16 & 15\_07\_11\_50\_00 \\
& IB & 200 & 273122 (358929) & 94153 (111986) & 5264 (8566) & - & 2000 (TO) & - & ... \\
\hline
\end{tabular}
\label{tab:spec1}
\end{center}
\end{table*}




\subsection{General \ac{MILP} Encoding}
\begin{itemize} [leftmargin=*]
    \item Linear predicate: each linear predicate is represented through a linear function $\mu(.)$. We use linear predicates to indicate whether \emph{a point} lies in the inside/outside face of an edge of a convex polygon $\mathcal{P}$ (see \eqref{eq:zpi_sdp}). For instance, let 
    ${\mu(p_i) = \frac{b^j - A^jp_i}{\norm{A^j}_2} \geq \epsilon}$ be a linear function. If $\mu(p_i) \geq 0$, $p_i$ lies \emph{inside} the edge $(A^j, b^j)$ of $\mathcal{P}$ with $\epsilon$ space margin. We can capture $\mu(p_i) \geq 0$  through a binary variable $b^{\mu}$ as
    \begin{flalign} \label{eq:milp_lin_pred}
    -M(1 - b^{\mu}) &\leq {\mu}(p_i) \leq Mb^{\mu} - m_\epsilon,
    \end{flalign}
    where $M, m_\epsilon$ are sufficiently large and small positive numbers respectively. If $b^{\mu} = 1$, ${\mu}(p_i) \geq 0$, else ${\mu}(p_i) < 0$. For the case ''\emph{outside} $(A^j, b^j)$ by $\epsilon$ space margin", we apply the same encoding method with ${\mu(p_i) = \frac{A^jp_i - b^j}{\norm{A^j}_2} \geq \epsilon}$. 

    \item Conjunction of $m$ binary variables, i.e., $b = \bigwedge_{i = 1}^m b_i$, is encoded through the following constraints
    \begin{nalign} \label{eq:conj_disj}
    b \leq b_i, \forall i \in \{1 \cdots m\} \text{ and } b \leq \sum_{i = 1}^m b_i - (m-1).
    \end{nalign}

    \item Disjunction of $m$ binary variables, i.e., $b = \bigvee_{i = 1}^m z_i$ is guaranteed with
    \begin{nalign} \label{eq:disj}
        b \geq b_i, \forall i \in \{1 \cdots m\}  \text{ and } b \leq \sum_{i = 1}^m b_i.
    \end{nalign}
    
    \item The infimum of $m$ continuous variables, i.e., $\binfmum_{i = 1}^m \theta_i$, is encoded through a continuous variables $\theta$ by introducing $m$ binary variables $\{b_1, \cdots, b_m\}$ and impose the following linear constraints
% \begin{nalign} \label{eq:min_enc}
%     \phi &= \bigwedge_{j = 1}^N \phi_i: \trob^{\phi} = \min ( \trob^{\phi_1},  \trob^{\phi_2}, \cdots  \trob^{\phi_N})\\
%     &\trob^{\phi_j} - (1 - b_j)M \leq \trob^{\phi} \leq \trob^{\phi_j} + (1 - b_j)M, \\ 
%     & ~\trob^{\phi} \leq \trob^{\phi_j} ~ \forall j \in \{1 \cdots N\}, ~\sum_{i = 1}^{N} b_j = 1
% \end{nalign}
% \begin{nalign} \label{eq:max_enc}
%     \phi &= \bigvee_{j = 1}^N \phi_i: \trob^{\phi} = \max (\trob^{\phi_1}, \trob^{\phi_2}, \cdots  
%     \trob^{\phi_N}) \\ 
%     &\trob^{\phi_j} - (1 - b_j)M \leq \trob^{\phi} \leq \trob^{\phi_j} + (1 - b_j)M, \\
%     & ~ \trob^{\phi} \geq \trob^{\phi_j}, ~ \forall j \in \{1 \cdots N\}, ~\sum_{i = 1}^{N} b_j = 1
% \end{nalign} 
    \begin{subequations} \label{eq:inf_sup}  
    \begin{align}        
        & \theta_i - (1 - b_i)M \leq \theta \leq \theta_i, \forall i \in \{1 \cdots m\}, \label{eq:inf_sup-a} \\ 
        &\sum_{i = 1}^{m} b_i = 1. \label{eq:inf_sup-b}
        \end{align}
    \end{subequations}
Equation \eqref{eq:inf_sup-a} ensures that $\theta$ is smaller than other variables and equal to any $\theta_i$ if and only if $b_i = 1$. Equation \eqref{eq:inf_sup-b} ensures that the infimum of the set exists. For supremum, we use the similar above encoding constraints, but replace \eqref{eq:inf_sup-a} with ${\theta_i \leq \theta \leq \theta_i + (1 - b_i)M}$.

\item {Multiplication  $y = xb, x \in \nSet{R}, b \in \nSet{B}$:} we impose
\begin{nalign} \label{eq:multi_xb}
  -Mb \leq y \leq Mb,~ x - M(1 - b) \leq y \leq x + M(1 - b),  
\end{nalign}
with positive $M$ is the sufficient large upper bound of $x$.
\end{itemize}

\subsection{{\tr} Encoding for \ac{PWL} signal}
\begin{itemize} [leftmargin=*]
 \item Atomic predicates $\pi / \neg \pi$ indicate whether a segment lies inside / outside of a region. These predicates are constructed from the conjunction and disjunction of linear predicates according to \eqref{eq:zpi_sdp}. We apply the above encoding strategy for linear predicates and logical operators \eqref{eq:milp_lin_pred}, \eqref{eq:conj_disj}, \eqref{eq:disj} to obtain the \emph{linear constraints} for $z_i^\lgPred$ and $z_i^{\neg\lgPred}$. With these constraints, these two binary variables $z_i^\lgPred$ and $z_i^{\neg\lgPred}$ that indicate whether segment $z_i$ satisfy/violate the atomic predicate $\lgPred$ or $\neg\lgPred$.

We use the right-time robustness $\rtrobzj{i}^{{\lgPred}}$ to explain the encoding. A similar strategy can be applied for the left time robustness. Let $\rtrobzj{i}^{{\lgPred}}$ be the right {\tr} of segment $z_i$ regarding $\lgPred$, we show how we can generate linear constraints such that $\rtrobzj{i}^{{\lgPred}}$ correspond to the definition of {\tr} in \eqref{eq:pwl_prop_tr_strict}. To this end, we adapt the "counting" encoding concept proposed by the authors in \cite{Rodionova2022TRTL} as follows.
%Recall the definition of $\rtrobzj{i}^{{\lgPred}}$ from \eqref{eq:pwl_prop_tr_strict}.
% Recall the definition of $\rtrobzj{i}^{{\lgPred}}$ as
% \hspace*{-0.75cm}\begin{nalign} \label{eq:ss}
%     \rtrobzj{i}^{{\lgPred}} &= \sign(z_i^{\lgPred}) \sum_{j = i+1}^{i + k}(t_{j+1} - t_j), \\ 
%     k &= \defkpeq \\
%     %
%     %\max_{\{0, 1, 2,\cdots, K\}} s.t. ~\forall i^\prime \in \{i+1, \cdots, i+k\}, \sign(z_i^{\lgPred}) = \sign(z^{\lgPred}_{i^\prime})\\
%     \rtrobzj{i}^{{\lgPred}} &= 0 \text{ if } k = 0.
% \end{nalign}
% Intuitively, if $z_i^{\lgPred} = \lgTrue$, we "aggregate" the time interval of the successive segment as long as these segments hold true regarding ${{\lgPred}}$. If the immediate successive segment doesn't hold, i.e., $z_{i+1}{\lgPred} = \lgFalse$, $z_i$ has $0$ right-{\tr}. Same explanation is applied for $z_i^{\lgPred} = \lgFalse$, but we have to multiply $-1$ additionally due to the sign operator $\sign(z_i^{\lgPred})$.
% In particular, they proposed the counting variables $c^1_i$ and $c^0_i$:  
% \begin{align} \label{eq:counting_milp}
%     c^1_i &= (c^1_{i+1} + 1)z_i, \\
%     c^0_i &= (c^0_{i+1} + 1)(1 - z_i).
% \end{align}
%
% We introduce the right-time robustness encoding for PWL segments wrt a proposition ${\lgPred}$ in the following. For any linear segment with timestamps $t_i, t_{i+1}$ and the symbolic binary variable $z_i$ determines the correctness of this segment wrt a proposition ${\lgPred}$, 
We first define the \emph{time-aggregating} variables $\Delta t^1_i$ and $\Delta t^0_i$ as below
\begin{nalign} \label{eq:t_aggre}
    \delta t_i &= t_{i+1} - t_i,\\ 
    \Delta t^1_i &= (\Delta t^1_{i+1} + \delta t_i)z_i^{\lgPred}, \\
    \Delta t^0_i &= (\Delta t^0_{i+1} - \delta t_i)(1 - z_i^{\lgPred}),
\end{nalign}
with ${\Delta t^1_{K-1} = \Delta t^0_{K-1} = 0}$. In the above formula, $\Delta t^1_i$
% From definition \ref{def:time_rob}, time robustness is defined as the strict time margin of the successive segments (not considering the interval of the current segment), we subtract this time amount from the variables defined in \eqref{eq:t_aggre}, i.e., 
% \begin{align*}
%     \Delta t^1_i &= \delta t^1_{i} - z_i\delta t_i \\
%     \Delta t^0_i &= \delta t^0_{i} + (1 - z_i)\delta t_i.
% \end{align*}
aggregates the time interval of the successive segments $z_{i+1}$ if $z^\lgPred_{i+1} = z^\lgPred_{i+1} = 1$, while  $\Delta t^0_i$ aggregate the negative time interval of $z_{i+1}$ if $z^\lgPred_{i+1} = z^\lgPred_{i+1} = 0$. Moreover, because \eqref{eq:t_aggre} is recursive, the aggregation continues until $z_{i+1} \neq z_{i}$. This corresponds to the sum operators used in \eqref{eq:pwl_prop_tr_strict}. 
In fact, the purpose of using two variables $\Delta t^1_i$ and $\Delta t^0_i$ is to distinguish the sign operator $\sign(z_i^\lgPred)$ defined in \eqref{eq:pwl_prop_tr_strict}. Since these variables are disjunctive, i.e., ${\Delta t^1_i \neq 0 \implies \Delta t^0_i = 0}$ and vice versa, the time robustness of one segment is 
% \begin{align}
%     \Tilde{\theta}^{{\lgPred}}_{+,i} = \Delta t^1_i  + \Delta t^0_i.
% \end{align}
\begin{subequations} 
\begin{align} 
   \rtrobzj{i}^{{\lgPred}} &= \Delta t^1_i  + \Delta t^0_i + \left(- z_i^{\lgPred}\delta_i + (1 - z_i^{\lgPred})\delta_i \right) \label{eq:tr_raw}\\ 
    &= z_i^{\lgPred}\Delta t^1_{i+1} + (1 - z_i^{\lgPred})\Delta t^0_{i+1} \label{eq:right_time_rob}
\end{align}
\end{subequations}
The last summand in \eqref{eq:tr_raw} is explained by the fact that the {\tr} defined in \eqref{eq:pwl_prop_tr_strict} does not contain the time interval $\delta_i$ of the current segment $z_i$.
% Finally, the time robustness is obtained by subtracting (or adding) the time interval of the current segments depending on $z_i^{\lgPred})$, i.e.,
% \begin{align} \label{eq:right_time_rob}
%     {\theta}^{{\lgPred}}_{+,i} &= \Tilde{\theta}^{{\lgPred}}_{+,i} - z_i^{\lgPred}\delta_i + (1 - z_i^{\lgPred})\delta_i \\ 
%     &= z_i^{\lgPred}\Delta t^1_{i+1} + (1 - z_i^{\lgPred})\Delta t^0_{i+1}
% \end{align}
To summarize, the time robustness $\rtrobzj{i}^{{\lgPred}}$ is encoded by introducing additional aggregating variables for each segment, then imposing linear constraints for the recursive formulas in \eqref{eq:t_aggre}, and also leverage \eqref{eq:multi_xb} to impose linear constraints that reflect the multiplication of binary and continuous variables as shown in \eqref{eq:right_time_rob}.  
%To express ${\theta}^{{\lgPred}}_{+,i}$ with linear constraints, the primary challenge is to encode \eqref{eq:t_aggre}, i.e., the multiplication of a continuous and a binary variable by using \eqref{eq:multi_xb}. 
% The primary encoding challenge for ${\lgPred}$ is to express $\eqref{eq:t_aggre}$ as linear constraints. This can be realized through the encoding strategy for the product of a continuous and binary variable $y = xb$, i.e., ${-Mb \leq y \leq Mb,~ x - M(1 - b) \leq y \leq x + M(1 - b)}$, with positive $M$ as the sufficient large upper bound of $x$.

% \begin{remark}
% Different from the discrete-time semantics, we don't subtract the time-interval of the current segment as shown in \cite{RodionovaTRTL} because $\delta t_i$ is already strict positive and considered as the time robustness of the segment $i$. 
% \end{remark}
% %
% \thought{
% \begin{remark}
% The time robustness is "counted" in   \cite{RodionovaTRTL} as can be seen in \eqref{eq:counting_milp}. In our "aggregating" encoding \eqref{eq:right_time_rob}, it is computed from the continuous time variables $t_i$. This may explain why DT could find a solution faster.
% \end{remark}
% }

\item {Temporal Operators:} For temporal operators, 
we need an indicator to check whether two segments $[t_{i1}, t_{i2}]$ and $[t_{j1}, t_{j2}]$ intersect. We use a $b^\intersect_{ij}$ boolean variable with linear constraints 
${b^\intersect_{ij} \lgEqual (t_{j2} - t_{i1} \geq \epsilon_t) \lgAnd (t_{i2} - t_{j1} \geq \epsilon_t) }$,  
where $\epsilon_t$ is non-negative. If $b^\intersect_{ij} = \lgTrue$, the intervals intersect, else they don't.
%
We instruct the encoding for the "eventually" ($\tlEvtll$), the other operators can be done similarly. Recall the definition from \eqref{eq:evtll_time_rob_strict}, let $\trob^*$ be $\trobzj{i}^{\stlEvtll{a,b}\lgSpec}$, we use $K-1$ additional binary variables $[b_1 \cdots b_{K-1}]$ that for each segment, then we impose the following linear constraints  
\begin{subequations} 
\begin{flalign}
& b_{ij}^\intersect \lgEqual [t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i + b] \neq \varnothing, t_{i+1} - t_i \leq b - a, \notag\\
& \trobzj{j}^\lgSpec - (1- b_{ij}^\intersect)M \leq \trob^*, \forall j \in \{1 \cdots K\}, \label{eq:geq_evtll_tr} \\
& \trob^* \leq \trobzj{j}^\lgSpec + (1- b_{j})M, \forall j \in \{1 \cdots K\}, \label{eq:evtll_tr_leq}\\  
& b_{ij}^\intersect \geq b_j, \forall j \in \{1 \cdots K\}; \sum_{j = 1}^K b_j = 1. \label{eq:supremum_exists}
\end{flalign}
\end{subequations} 
In the above constraints, the \eqref{eq:geq_evtll_tr} implies that $\trob^*$ is greater or equal to the time robustness of \emph{any} segments that intersect with $[t_{i+1} +a, t_i + b]$. Meanwhile, \eqref{eq:evtll_tr_leq} guarantees that $\trob^*$ is bounded by $\trobzj{j}^\lgSpec$ whenever $b_{j} = 1$. Finally, \eqref{eq:supremum_exists} ensures that the supremum belongs to the given set that intersects, i.e, $b_j = 1 \implies b_{ij}^\intersect = 1$, and $\sum_{j = 1}^K b_j = 1$ ensures that there exists one segment with the maximal time robustness (supremum).
\end{itemize}

% Similarly for the "always" operator, recall the definition from \eqref{eq:alws_time_rob_strict} and let $\trob^*$ be $\trobzj{i}^{\stlAlways{a,b}\lgSpec}$, we impose the following constraints
% \begin{flalign*}    
% &\trobzj{j}^\lgSpec - (1- b_{j})M \leq \trob^* \leq \trobzj{j}^\lgSpec + (1- b_{ij}^\intersect)M, ~ \forall j \in \{1 \cdots K\},\\ 
% & b_{ij}^\intersect = [t_j, t_{j+1}] \intersect [t_{i} +a, t_{i+1} + b] \neq \varnothing, b_{ij}^\intersect \geq b_j, \sum_{j = 1}^K b_j = 1. 
% \end{flalign*}
% \thought{
% \begin{remark}
% Did we introduce any conservatism here?
% \end{remark}
% }
% The encoding for the "until" operator is performed similarly. 
% % \begin{align*}
% %     \trob^{\phi_1\stlUntil{a,b}\phi_2}(z_i) &= \max_{j \in \set{J}^\intersect}\left( \min \left( \trob^{\phi_2}(z_j), \min_{l \in \set{L}_j^\intersect}\trob^{\phi_1}(z_l) \right)\right), \\
% % \set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \set{L}^\intersect_j = \left\{1 \cdots j | b^\intersect_{il} = 1\right\}, \\
% % b^\intersect_{ij} &= ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing, \\
% % b^\intersect_{il} &= [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing.
% % \end{align*}
% Let $\trobzj{i}^*$ be the {\tr} of the until operator that we want to derive. To encode the inner $\min$ operator, we denote them as $K$ continuous variables
% \begin{align*}    
% &[\underline{\trobzj{1}}, \cdots, \underline{\trobzj{K}}] = [{\min_{l \in \set{L}_1^\intersect}(\trobzj{1}^{\phi_2}, \trobzj{l}^{\phi_1}}), \cdots ,{\min_{l \in \set{L}_K^\intersect}(\trobzj{K}^{\phi_2}, \trobzj{l}^{\phi_1}})], 
% \end{align*}
% where ${\set{L}^\intersect_j = \left\{1 \cdots j | b^\intersect_{il} = ([t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing) =  1\right\}}$. Recall that the time intersection set of the outer $\max$ operator is defined as ${\set{J}^\intersect = \left\{1 \cdots K | b^\intersect_{ij} = ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing) 
%  = 1\right\}}$, we rewrite the time robustness of the "until" operator as follows.
% \begin{flalign*}
% & \forall j \in \{1 \cdots K\}, b^\intersect_{ij} = 1 \hequal \forall j \in \set{J}^\intersect \implies \trobzj{i}^* \geq \underline{\trobzj{j}}, \\
% & \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2} \lgAnd \left(\forall l \in \{1 \cdots j\}, b^\intersect_{il} = 1 \hequal \forall l \in \set{L}^\intersect_j \implies (\underline{\trobzj{j}} \leq \trobzj{l}^{\lgSpec_1})\right).
% \end{flalign*}
% For each $\underline{\trobzj{j}} = \min_{l \in \set{L}_j^\intersect (\trobzj{j}^{\phi_2}, \trobzj{l}^{\phi_1}})$, we use $j+1$ additional binary variables $[\bmin{1}^j, \bmin{2}^j, \cdots, \bmin{j}^j, \bmin{j+1}^j]$ with $\sum_{l = 1}^{j+1} \bmin{l}^j = 1$ and impose the following constraints
% \begin{nalign}
% & \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2}, \trobzj{j}^{\lgSpec_2} - (1- \bmin{j+1}^j)M \leq \underline{\trobzj{j}} \leq \trobzj{j}^{\lgSpec_2} + (1- \bmin{j+1}^j)M,\\ 
% & \forall l \in \{1 \cdots j\}, b_{il}^\intersect \geq \bmin{l}^j, \trobzj{l}^{\lgSpec_1} - (1- \bmin{l}^j)M \leq \underline{\trobzj{j}} \leq \trobzj{l}^{\lgSpec_1} + (1- b_{il}^\intersect)M.\\
% \end{nalign}
% Afterwards, we encode the outer $\max$ operators considering time intersection, we introduce $K$ additional binary variables $[\bmax{1}, \bmax{2} \cdots \bmax{K}]$ with $\sum_{j = 1}^K \bmax{j} = 1$ and impose the following constraints for all $j \in \{1 \cdots K\}$
% \begin{flalign*}
% & \underline{\trobzj{j}} - (1- b^\intersect_{ij})M \leq \trobzj{i}^* \leq \underline{\trobzj{j}} + (1- \bmax{j})M, ~b^\intersect_{ij} \geq \bmax{j}. 
% \end{flalign*}

\subsection{Complexity Analysis} \label{sec:complex_ana}
Each convex region with $m$ edges is represented through $m$ linear predicates. For a \ac{PWL} signal consists of $K$ segments, the qualitative encoding complexity of atomic predicates and its negation is $\bigO(mK)$ (or $\bigO(K)$). To encode the {\tr}, we need $\bigO(K)$ additional continuous variables as shown in \eqref{eq:t_aggre}. 
%For qualitative $\pi$ and $\neg\pi$, each segments requires $2m$ predicates. Thus the whole path needs $\bigO(2mK)$ or $\bigO(K)$ if $m$ is not significant. {\tr} encoding introduces $\bigO(K)$ additional continuous variables. 
For each temporal operator, each segment needs $\bigO(K)$ additional binary and $\bigO(1)$ continuous variables for infimum/supremum encoding, which respectively results in $\bigO(K^2)$ and $\bigO(K)$ for the whole signal with $K$ segments \footnote{However, for a formula with \emph{one single temporal operator}, e.g., $\stlEvtll{I} {\lgPred}$, $\stlAlways{I} {\lgPred}$, we just impose constraints on the first segment, thus only requiring $\bigO(|\lgSpec|K)$ binary variable.}.  
In summary, the generalized complexity to encode any STL formula $\lgSpec$ with $|\lgSpec|$ is a number of temporal operators, the number of variables to be solved with \ac{MILP} is $\bigO(|\lgSpec|K)$ continuous variables and $\bigO(|\lgSpec|K^2)$ binary variables. Compared to the instance-based signal with $T$ instances, the complexity shown in \cite{Rodionova2022TRTL} is $\bigO(|\lgSpec|T)$ binary and continuous variables. Although using \ac{PWL} signal has the quadratic term $K^2$ complexity, various path-planning problems can be represented in practice with $K^2 \ll T$. Moreover, we observe that the complexity \emph{does not depend on $T$}, which makes the usage of \ac{PWL} signal advantageous for long-time horizon planning problems.


==> sections/discussion.tex <==
\section{Discussion}

\subsection{Strict vs Modified Encoding}

\subsection{MILP GAP does not close for some specification}

\begin{nalign}
    \stlEvtll{0, 10} \stlAlways{3, 7} \pi \\
    \stlEvtll{0, 10} \stlAlways{0, 5} \pi    
\end{nalign}


\subsection{Why Modified PWL Encoding}
The authors in \cite{Sun20223451} proposed the qualitative encoding for PWL trajectory. We note that the encoding imposes unnecessary constraints. In particular,
\begin{itemize}
    \item For each encoding starting from $j$, it is sufficient to impose constraints on the successive segments, not the whole trajectory. \item For the time intersection from temporal operators, it is sufficient to use the starting time of each segment, not both the starting and ending time.
\end{itemize}

The qualitative semantics depends on the "Until" operator that is rewritten below
\begin{nalign} \label{eq:rw_bool_pwl_until}
    z_{i}^{\lgSpec_1\stlUntil{a,b}\lgSpec_2} &: \exists t^\prime \in [t_{i} + a, t_i +b], \\
    & \hspace*{-1cm} \bigvee_{j = i}^{K} \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec_2} \lgAnd \bigwedge_{l = i}^j \left(t^\prime \in [t_l, t_{l+1}] \implies z_l^{\lgSpec_1}\right)\right)
\end{nalign}
The equivalent semantics for "eventually" and "always" are obtained
\begin{nalign} \label{eq:rewritten_fml}
    z_{i}^{\stlAlways{a,b}\lgSpec} &= \bigwedge_{j = i}^{K} \left([t_j, t_{j+1}] \intersect [t_{i} + a, t_{i} + b] \neq \varnothing \implies z_j^\lgSpec \right) \\
    %
    z_{i}^{\stlEvtll{a,b}\lgSpec} &= \bigvee_{j = i}^{K} \left([t_j, t_{j+1}] \intersect [t_{i} + a, t_{i} + b] \neq \varnothing \lgAnd z_j^\lgSpec \right) \\
    %
    z_{i}^{\lgSpec_1\stlUntil{a,b}\lgSpec_2} &= 
    \bigvee_{j = 1}^{K} \Big(([t_j, t_{j+1}] \intersect [t_{i} +a, t_i +b] \neq \varnothing \lgAnd z_j^{\lgSpec_2}) \\
    & \lgAnd \bigwedge_{l = 0}^j ([t_l, t_{l+1}] \intersect [t_{i}, t_{i} +b] \neq \varnothing \implies z_l^{\lgSpec_1})\Big) \\ 
    %    
    % z_k^{\varphi_1 \stlUntil{a,b} \varphi_2} &= \lgAnd_{k = 0}^{H - 1} \left([t_j, t_{j+1}] \cup [t_i + a, t_{i+1} + b] \right) \\
\end{nalign}


\subsection{Heuristics and Prediction}

\begin{itemize}
    \item Pre-allocate timestamps
    \item 
\end{itemize}


\subsection{Loss of Negation}
\begin{remark}  \label{rem:pwl_lost_negation}  
    To be clear, the explicit definition of the above atomic predicates results in the loss in negation formula, i.e.,
    \begin{nalign}
      z_i^{{\lgPred}} \neq \lgNeg z_i^{{\lgNeg\pi^{\mu}}}  
    \end{nalign}
    It can be derived from \eqref{eq:sdp_pwl} and \eqref{eq:zpi_sdp} that we only have the following sufficient conditions ${z_i^{{\lgPred}} = \lgTrue \implies z_i^{{\tlNot\pi^{\mu}}} = \lgFalse}$ and $z_i^{{\tlNot\pi^{\mu}}} = \lgTrue \implies z_i^{{\lgPred}} = \lgFalse$. We \emph{do not} have ${z_i^{{\lgPred}} = \lgFalse \implies z_i^{{\tlNot\pi^{\mu}}} = \lgTrue}$ or ${z_i^{{\tlNot\pi^{\mu}}} = \lgFalse \implies z_i^{{\lgPred}} = \lgTrue}$. Such a situation occurs, for instance, when a segment intersects with a region. 
\end{remark}


\subsection{Time-Robustness STL}
We first introduce the time-robustness semantics for instance-based signal studied in \cite{Donze2010RSTL, RodionovaTRTL}. Then, we formulate and clarify the definition of time robustness considering \ac{PWL} trajectory for the atomic predicate and each temporal operator according to the aforementioned STL syntax \eqref{eq:stl_syntax}.
%  The \emph{spatial robustness} $\rho^{\pi^\mu}(x)$ is then defined as "how much" a signal fulfills an STL formula according to the following recursive rule 

% \begin{definition}[Space Robustness \cite{Donze2010RSTL}] \label{def:time_rob}
% \begin{align}
%     \rho^{{\pi^\mu}}(\xi, t) &= \mu(\xi(t)) \\
%     \cdots 
% \end{align}
% \end{definition}
% \thought{Actually, I think we don't need to remind the spatial robustness here.}

\thought{I agree with you that this section is not relevant to our work. Where should we move it?}
\begin{definition}[Time Robustness \cite{Donze2010RSTL}] 
The right/left time robustness indicates the time margin that the signal can be shifted right/left and still maintains its characteristic related to a given specification, i.e.,
\newcommand \sgnxit{\sign(\xi_t^{{\pi^\mu}})}
\newcommand \sgnxitp{\sign(\xi_{t^\prime}^{{\pi^\mu}})}

\small
\begin{nalign}
\theta_+^{{\pi^\mu}}(\xi,t) &= \sgnxit.\max\{\tau \geq 0: \forall t^\prime \in [t, t+ \tau], \sgnxit = \sgnxitp\}, \\ 
% Neg
\theta_-^{{\pi^\mu}}(\xi, t) &= \sign(\xi_t^{{\pi^\mu}}).\max\{\tau \geq 0: \forall t^\prime \in [t - \tau, t], \sgnxit = \sgnxitp\}. 
\end{nalign}
\normalsize
%  with ${\mu(\xi(t)) \overset{{\pi^\mu}}{\equiv} \mu(\xi(t^\prime))} \hequal {\mu(\xi(t)) \lgSatisfy {\pi^\mu} \iff \mu(\xi(t^\prime)) \lgSatisfy {\pi^\mu}}$.
% The expression ${\mu(\xi(t)) \overset{{\pi^\mu}}{\equiv} \mu(\xi(t^\prime))}$ can also be formulated through the sign function as follow \cite{RodionovaTRTL}
% \[\mu(\xi(t)) \overset{{\pi^\mu}}{\equiv} \mu(\xi(t^\prime)) \iff \sign(\mu(\xi(t))) = \sign(\mu(\xi(t^\prime))),\]
% where the sign function is defined as 
% \begin{nalign}
%     \sign(x): \nSet{R} \xrightarrow{} \{-1,0,1\} = 
%     \begin{cases}
%         1 & x > 0 \\
%         0 & x = 0 \\
%         -1 & x < 0
%     \end{cases}, \\
%     \sign(x): \{0,1\} \xrightarrow{} \{-1,1\} = 
%     \begin{cases}
%         1 & x = 1 \\
%         -1 & x = 0
%     \end{cases}    
% \end{nalign}
\end{definition}
For other formulas and temporal operators in \eqref{eq:stl_syntax}, the quantitative semantic is defined recursively below.
\begin{definition}[Time-Robustness STL Semantics \cite{Donze2010RSTL}] \label{def:quanti_tr}
\begin{nalign}
    \trob^{\lgNeg\lgSpec}(\xi, t) &=  - \trob^{\lgSpec}(\xi, t) \\ 
    \trob^{\lgSpec_1 \lgAnd \lgSpec_2}(\xi, t) &= \trob^{\lgSpec_1}(\xi, t) \infmum \trob^{\lgSpec_2}(\xi, t) \\
    \trob^{\lgSpec_1 \lgOr \lgSpec_2}(\xi, t) &= \trob^{\lgSpec_1}(\xi, t) \supmum \trob^{\lgSpec_2} (\xi, t) \\
    \trob^{\lgSpec_1 \stlUntil{a,b} \lgSpec_2}(\xi, t) &=  \bsupmum_{t^\prime \in [t+a, t+b]}\left(\trob^{\lgSpec_2}(\xi, t^{\prime}) \infmum \binfmum_{t^{\prime\prime} \in [t, t^\prime)} \trob^{\lgSpec_1}(\xi, t^{\prime\prime}) \right), 
\end{nalign}
where the notation $\theta_{\bowtie}^{\lgSpec}$ indicates either right or left time robustness, i.e., ${\bowtie = \{+,-\}}$. 
\end{definition}


\subsection{Strictness of the encoding from IB perspectives}
\begin{nalign} \label{eq:sdp_pwl}
 %z^\lgSpec_i & \lgEqual z_i \lgSatisfy \lgSpec,\\ 
 z^\lgSpec_i &= \lgTrue \iff \sign(z^\lgSpec_i) = 1 \iff \forall t \in [t_i, t_{i+1}], (\xi, t) \lgSatisfy \lgSpec, \\
 z^\lgSpec_i &= \lgFalse \iff \sign(z^\lgSpec_i) = -1 \iff \exists t \in [t_i, t_{i+1}], (\xi, t) \not\lgSatisfy \lgSpec.
\end{nalign}
Intuitively, the above property ensures that if a segment satisfies a formula $\lgSpec$, all of the signal instances within that segment also satisfy $\lgSpec$. 

\thought{The relation of the above notation to the instance-based syntax can be seen from \eqref{eq:sdp_pwl}, i.e, 
\begin{align*}
     z^\lgSpec_i &= \lgTrue \iff \sign(z^\lgSpec_i) = 1 \iff \forall t \in [t_i, t_{i+1}], (\xi, t) \lgSatisfy \lgSpec, \\
     \trobzj{i}^\lgSpec &= \binfmum_{t \in [t_i, t_{i+1}]} \trob^{{\lgSpec}}(\xi, t) 
\end{align*}
We want to have a strong encoding property, i.e., 
\begin{nalign}
    \trobzj{i}^\lgSpec > 0 \implies \trob^{{\lgSpec}}(\xi, t), ~\forall t \in [t_i, t_{i+1}]. 
\end{nalign}
Read: the time robustness of a \emph{segment} is the \emph{minimum} time robustness of \emph{every} time instance of that segment. 
 }
 \critical{This property is for me the most reasonable reason that the optimization problem is harder to be solved. You can see the Remark in section III-A in \cite{Sun20223451}.}

 \subsection{Loss of Negation}
 \thought{
From Remark \ref{rem:pwl_lost_negation} we show that don't have both necessary and sufficient conditions for \emph{negation}, which means we don't have $\trobzj{i}^{\lgNeg\pi^\mu} =  - \trobzj{i}^{\pi^\mu}$ We can only show that $\trobzj{i}^{\lgNeg\pi^\mu} > 0 \implies \trobzj{i}^{\pi^\mu} < 0$ and $\trobzj{i}^{\pi^\mu} > 0 \implies \trobzj{i}^{\lgNeg\pi^\mu} < 0$, not $\trobzj{i}^{\lgNeg\pi^\mu} < 0 \implies \trobzj{i}^{\pi^\mu} > 0$, and not $\trob^{\pi^\mu} < 0 \implies \trobzj{i}^{\neg\pi^\mu} > 0.$  
}

\subsection{Physical Meaning - nice property of time-robustness}
\thought{For instance-based trajectory, the following property is straightforwardly observed. It is a nice property, but I am not sure if we should claim and prove it?}
Similar to Theorem 2 in \cite{Donze2010RSTL}, we have the following property from the above definition
\begin{property}[Strict-Time Robustness]
Regards any STL formula $\lgSpec$ and the signal $z_i$, if $\trob^{\lgSpec}(z_i) = \tau$ is the right (left) time robustness, then for any signal $z_i^\prime$ obtained from shifting $z_i$ left (right) by less than $\tau$, we have $\sign(z^\lgSpec_i) = \sign(z^\lgSpec_{i^\prime})$.
\end{property}


\thought{
\begin{remark} [Strictness of the encoding]
    blah blah ...
\end{remark}
}


==> sections/evaluation.tex <==
\section{Benchmark} \label{sec:bm}
% \begin{figure}[t]
% \begin{multicols}{2}
%     \subfloat[$\lgSpec_1$ Multi-Blocks-1
%       \label{fig:exp-a}]{\includegraphics[width = 0.23\textwidth]{figs/monitor_target_1.png}} \hfill \par
%     %\caption{Multi-Blocks}
%     \subfloat[$\lgSpec_2$ Multi-Blocks-2
%       \label{fig:exp-b}]{\includegraphics[width = 0.23\textwidth]{figs/Multi_Random_0.png}} \hfill \par
%     \subfloat[$\lgSpec_3$ Door-Puzzle-1
%       \label{fig:exp-dp1}]{\includegraphics[width = 0.23\textwidth]{figs/DoorPuzzle1.png}} \hfill \par
%     \subfloat[$\lgSpec_4$ Door-Puzzle-2
%       \label{fig:exp-dp2}]{\includegraphics[width = 0.23\textwidth]{figs/DoorPuzzle2.png}} \hfill \par
% \end{multicols}
\begin{figure}[t]
% \begin{multicols}{2}
%     \subfloat[$\lgSpec_1$ Multi-Blocks-1
%       \label{fig:exp-a}]{\includegraphics[width = 0.23\textwidth]{figs/result/MB1_fig.png}} \hfill \par
%     %\caption{Multi-Blocks}
%     \subfloat[$\lgSpec_2$ Multi-Blocks-2
%       \label{fig:exp-b}]{\includegraphics[width = 0.24\textwidth]{figs/result/MB2_14_00_29.png}} \hfill \par
%     \subfloat[$\lgSpec_3$ Door-Puzzle-1
%       \label{fig:exp-dp1}]{\includegraphics[width = 0.25\textwidth]{figs/result/K23_DP1_fig.png}} \hfill \par
%     \subfloat[$\lgSpec_4$ Door-Puzzle-2
%       \label{fig:exp-dp2}]{\includegraphics[width = 0.25\textwidth]{figs/result/DP2_12_33_07_mod.png}} \hfill \par
% \end{multicols}
\begin{multicols}{2}
    \subfloat[$\lgSpec_1$ Multi-Blocks-1
      \label{fig:exp-a}]{\includegraphics[width = 0.23\textwidth]{figs/replot_result/MB1_fig_grid_major.png}} \hfill \par
    %\caption{Multi-Blocks}
    \subfloat[$\lgSpec_2$ Multi-Blocks-2
      \label{fig:exp-b}]{\includegraphics[width = 0.24\textwidth]{figs/replot_result/MB2_12_54_52_major.png}} \hfill \par
    \subfloat[$\lgSpec_3$ Door-Puzzle-1
      \label{fig:exp-dp1}]{\includegraphics[width = 0.25\textwidth]{figs/replot_result/DP1_fig_grid_major.png}} \hfill \par
    \subfloat[$\lgSpec_4$ Door-Puzzle-2
      \label{fig:exp-dp2}]{\includegraphics[width = 0.25\textwidth]{figs/replot_result/DP2_grid_major.png}} \hfill \par
\end{multicols}
\caption{Experiment results of four scenarios with different complexity. In each figure, the blue dots are the synthesized waypoints. The \ac{PWL} signal is the blue piecewise-linear connecting the waypoints. The $XY$ plane consists of the reach (green/dark blue)-avoid (red/yellow) regions. The $Z$ axis denotes the synthesized time-stamp in seconds. The starting and ending positions are the declared markers as shown in the figures' legends.}
\end{figure}

\subsection{Experiment Setup}
%The experiments are performed on a Lenovo ThinkCentre M75-q2-gen2 computer with AMD Ryzen 7 4750GE, 3.1 Ghz, 16 Gb RAM, and running Linux OS. We use YALMIP \footnote{YALMIP - "https://yalmip.github.io/"} and MATLAB \footnote{MATLAB 2022b - "https://www.mathworks.com"} to implement the \ac{MILP} encoding. The optimization solver is Gurobi \footnote{Gurobi 10.0.1 - "https://www.gurobi.com"}. The numerical experiment uses {four} scenarios to verify: 1) the soundness of the encoding 2) the computational complexity 3) the sensitivity of the optimization. We also implement the \ac{IB} (IB) methods used in \cite{Rodionova2022TRTL} to compare the performance. To make the comparison fair, both methods are implemented in a similar hierarchical fashion. For IB method, we let the time step between each instance be $1 s$. The two algorithms are tested with the same task-dependant planning time horizon $T$ and limited velocity of $1 m/s$. For \ac{PWL} signal, we increase the number of waypoints $K$ incrementally until a feasible solution exists, and further increase $K$ to evaluate the sensitivity.
The numerical experiment uses {four} scenarios to verify: 1) the soundness of the encoding; 2) the computational complexity; and 3) the sensitivity of the optimization. We also implement the \ac{IB} method of \cite{Rodionova2022TRTL} to compare the performance \footnote{The implementation information is provided in Appendix \ref{apx:hw_info}}. To make the comparison fair, both methods are implemented similarly hierarchically. For the \ac{IB} method, we let the time step between each instance be $1 s$ so the planning horizon $T$ is also the number of instances. We emphasize the complexity analysis by choosing missions with short planning horizon ($T \ll K^2$), and when they are approximately equal ($T \approx K^2$), which is also sufficient to capture the long planning horizon case ($K^2 \ll T$). The two algorithms are tested with the same task-dependant planning time horizon $T$ and limited velocity of $1 m/s$. For \ac{PWL} signal, we increase the number of waypoints $K$ incrementally until a feasible solution exists, and further increase $K$ to evaluate the sensitivity.
%
The missions are chosen with different spatial and temporal complexity. To simplify the notation, temporal operators without time subscripts imply the overall time horizon $[0, T]$, e.g., ${\tlEvtll \hequal \stlEvtll{0, T}}$. The first two reach-avoid scenarios require a robot to perform a ``monitoring" task, i.e., visit a region and stay there for a certain time, while avoiding the red regions all the time, i.e., ${\lgSpec_1 = \bigwedge_{i = 1}^{8} \lgNeg A_i \lgAnd  \tlEvtll \stlAlways{0,5} R_1  
\lgAnd \tlEvtll\stlAlways{0, 5} R_2}$. The starting and ending position is given. 
% \begin{align*}
%     \lgSpec_1 = & {\bigwedge_{i = 1}^{20} \lgNeg A_i \lgAnd  \tlEvtll \stlAlways{0,5} R_1  
%     \lgAnd \tlEvtll\stlAlways{0, 5} R_2 \lgAnd \tlEvtll \stlAlways{0, 5} R_3}
% \end{align*}
The second one uses a longer time horizon $T_{\max} = 300$. One additional region must be monitored with an explicitly given time window, i.e., $\lgSpec_2 = \bigwedge_{i = 1}^{20} \lgNeg A_i \lgAnd  \stlEvtll{0, 150}\stlAlways{0,15} R_1  \lgAnd \stlEvtll{180, 260}\stlAlways{0, 15} R_2  
\lgAnd \stlEvtll{50,80}\stlAlways{0, 15} R_3 \lgAnd \stlAlways{200, 220} R_3 $
% \begin{align*}    
%     \lgSpec_2 = & \bigwedge_{i = 1}^{20} \lgNeg A_i \lgAnd  \stlEvtll{0, 150}\stlAlways{0,15} R_1  \lgAnd \stlEvtll{180, 260}\stlAlways{0, 15} R_2 \\ 
%     & \lgAnd \stlEvtll{50,80}\stlAlways{0, 15} R_3 \lgAnd \stlAlways{200, 220} R_3 
% \end{align*} 
In the third scenario, the robot eventually visits region $R_1$ and stay there at a certain time window. Region $R_2$ should be eventually visited, but the robot is not allowed to pass through the yellow gate $G_1$ before reaching the charging area $C_1$, i.e, ${{\lgSpec_3 = \neg G_1\stlUntil{0, 30} C_1 \lgAnd \stlEvtll{50,80}\stlAlways{0,5}R_1 \lgAnd \tlEvtll\stlAlways{0,5}R_2}}$.
% The fourth scenario shows a surveillance task with a specified order. The robot is required to visit R3 in a specified time interval, then R2, and finally R1. The executed path length and the right-time robustness of these formulas are optimized. The encoding is written as ${{\lgSpec_3 = \bigwedge_{i = 1}^{10} \tlAlways\neg A_i \lgAnd \stlEvtll{0, 30} R_1 \lgAnd \stlEvtll{30,60} R_2 \lgAnd \stlEvtll{60,80} R_3}}$.
%
The fourth scenario tests the exhaustive search of the encoding to solve the puzzle taken from \cite{Sun20223451}. The robot is not allowed to pass through the gates until the key with a corresponding number is collected at the green region. The final goal is to reach the blue region, i.e., 
${\lgSpec_4 = \tlEvtll G \lgAnd (\lgAnd_{i=1}^5 \tlAlways \lgNeg A_i) \lgAnd \lgAnd_{i=1}^5 \lgNeg D_i \tlUntil R_i}$.
% \begin{itemize}
%     \item Reproduce the previous work of \cite{RodionovaTRTL} - Altitude Control
%      {${\lgSpec_1 = \stlAlways{20,30} (z \geq 20) \lgAnd \stlAlways{60,70} (z \leq 10)}$}
%       \item Door-Puzzle-1
%     \[\lgSpec_2 = \neg G_1\stlUntil{0, 30} C_1 \lgAnd \stlEvtll{50,80}\stlAlways{0,5}R_1 \lgAnd \stlEvtll{0,T}\stlAlways{0,5}R_2\]
%     \item Sequential Multi-Blocks.
%      \[\lgSpec_3 = \bigwedge_{i = 1}^{10} \stlAlways{0,T}\neg A_i \lgAnd \stlEvtll{0, 30} R_1 \lgAnd \stlEvtll{30,60} R_2 \lgAnd \stlEvtll{60,80} R_3\]
%      \item Sequential Multi-Blocks.
%      \begin{nalign}
%      & \lgSpec_3^\prime = \bigwedge_{i = 1}^{10} \stlAlways{0,T}\neg A_i \lgAnd \stlEvtll{150, 180}\stlAlways{0,20} R_1 \lgAnd \\  & \stlEvtll{0,180}\stlAlways{0, 20} R_2 \lgAnd \stlEvtll{0,80}\stlAlways{0, 20} R_3
%      \end{nalign}
%      Impose constraints: each monitoring task has right-time robustness larger than 5. Objectives: Maximizing right-time-robustness of the region $R_3$.
%
%     \item Multi-Blocks-2 
%     \begin{nalign} \label{eq:spec_4}
%         \lgSpec_4 = &\bigwedge_{i = 1}^{20} \lgNeg A_i \lgAnd \stlEvtll{0, 80}\stlAlways{0,5} R_1 \\ 
%         \lgAnd & \stlEvtll{0,80}\stlAlways{0, 5} R_2 \lgAnd \stlEvtll{0,80}\stlAlways{0, 5} R_3
%     \end{nalign}
%     Maximizing $\theta_{R_1}$ and minimizing path length. Each sub specification is required to have 3 s time robustness
%
%     \item Reach-Avoid Simple
%     \item Reach-Avoid Multi Avoid Regions
%     \item Reach-Avoid Sequential
%     \item Puzzle - "Until" Operator
%     \item Surveillance and Charging
%     \item Multi-Agent Collision Avoidance 
%     \item Multi-Agent Multi Target
% \end{itemize}
%\thought{Briefly described the objective. The objects can be weighted path length and time robustness, or we set the time robustness greater equal a threshold as a linear constraint.} 
All scenarios are optimized by maximizing the time-robustness and minimizing the path length with $\lambda = 1$. 

\subsection{Experiment Result}
Table \ref{tab:bm} shows the encoded \ac{MILP}'s information and the optimization results. 
%We evaluate the results below to clarify the 
%. The methods are distinguished by the number of segments $K$ (\ac{PWL}) and the time-horizon $T$ (\ac{IB}) respectively. The "MILP Info" column shows the size of the model: the number of constraints (\# Cstr), binary variables (\# Bin), and continuous variables (\# Cont). The value of the objective (Obj.) is $(L, \theta_+)$ is the path length and time-robustness in seconds. The last column shows the optimization time of Gurobi, where the number denoted with the symbol $*$ is the time that the solver converges to the optimal objective. We also let the solver search over the complete solution space and recorded the solving time.
%\thought{We might omit this! In these columns, we provide the number of variables of constraints before and after being resolved by Gurobi (the number inside the brackets is the original number before the presolver)}. 
%The solving time consists of Yalmip time to build the model, and the solving time of Gurobi. We use the default configuration for Gurobi. 
\begin{enumerate} [leftmargin=*]
    \item \emph{Soundness}: overall, all obtained solution is sound, i.e., none of them violates the imposed specification.

    \item \emph{Model Complexity}: the size of the \ac{MILP} corresponds to the complexity analysis in Section \ref{sec:complex_ana}. Compared to the IB approach, we summarize our observations below
    \begin{itemize} [leftmargin=*]
        \item The encoding complexity depends on $K$, i.e., the required numbers of continuous and binary variables are $\bigO (|\lgSpec|K^2)$ and $\bigO (|\lgSpec|K)$ respectively. This is best observed when we vary $K$ in $\lgSpec_1$ and $\lgSpec_3$.  
        \item Encoding with \ac{PWL} signal requires fewer continuous variables (all four scenarios).
        \item For short planning horizon ($T \ll K^2$), \ac{PWL} signal requires more binary variables due to the quadratic $\bigO (|\lgSpec|K^2)$ (see $\lgSpec_1$ and $\lgSpec_3$). 
        However, in $\lgSpec_2$ and $\lgSpec_4$, \ac{PWL} encoding requires fewer binary variables because these formulas are dominated by a large number of sub-formulas with one single temporal operator, which was explained in the footnote of Section \ref{sec:complex_ana}.
    \end{itemize} 
    \item \emph{Objectives and Sensitivity Analysis}: in our algorithm, the objective depends on $K$. Consider $\lgSpec_3$, we need at least 23 waypoints to obtain a feasible solution. When we increase $K = 25$, another solution with better time-robustness is found. In fact, with more waypoints, the solution space is larger and may contain a better solution. 
    %Figure \critical{X} confirms the explanation by showing that additional segments allow the signal to pass through the narrow corridors which saves time for other tasks. 
    Nevertheless, further increasing $K$ \emph{do not} always improve the solution, which is observed when we further increase $K$ to 30, or through the results of $\lgSpec_1$.  

    \item \emph{Computation Time}: the solving time does not depend solely on the number of constraints and variables. With greater $K$, \ac{MILP} requires a longer time to obtain a feasible solution and in many cases \emph{much longer time} to completely terminate the program. We hypothesize that it is affected by the large feasible solution space. Since we are maximizing the time robustness directly through the continuous timestamps, it is hard for the branch-and-bound methods to determine the optimal search path. Further investigation is needed in future work.     
  \end{enumerate}
  
% & PWL & K & cstr (-) & bin (-) & cont (-) & obj & grb & ym & notes \\
% & IB & T & cstr (-) & bin (-) & cont (-) & obj & grb & ym & notes \\
\begin{table}    
\begin{center}
%\caption{BENCHMARK}
%\hspace*{-0.45cm}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 %\multicolumn{7}{|c|}{$\lgSpec = \stlAlways{20,30} (z \geq 20) \lgAnd \stlAlways{60,70} (z \leq 10)$} \\
 %\hline
%\multirow{1}{*}{Type}
 
\multicolumn{1}{|c|}{Methods} &\multicolumn{4}{|c|}{MILP Info} & \multicolumn{1}{|c|}{Time [s]} \\
 \hline 
\textbf{PWL}/IB &\# Cstr & \# Bin & \# Cont & Obj ($L, \theta_+$) & GRB \\
% HBLT
% \hline
% \multirow{2}{*}{$\lgSpec$} 
% & PWL & K & cstr (-) & bin (-) & cont (-) & obj & grb & ym & Notes \\
% & IB  & T & cstr (-) & bin (-) & cont (-) & obj & grb & ym & notes \\
% % UAV
% \hline
% \multirow{2}{*}{$\lgSpec_1$} 
% & PWL & 23 & 652 & 146 & 95 & $\theta_+$ = 22 & 0.9 & 3.5 &\\
% & IB & 100 & 2447 & 224 & 502 & $\theta_+$ = 23 & 1.5 & 0.58&\\
% MB1
\hline
\hline
%\multirow{3}{*}{$\lgSpec_1$}
%\multicolumn{7}{|c|}{] \\
\multicolumn{6}{|c|}{$\lgSpec_1$} \\
\hline
%\multirow{3}{*}{$\lgSpec_1$}
\textbf{K = 23} &  22740 & 7724 & 895 & 44.7, 21.8 & 14* %\footnote{Symbol $*$ denotes the time that the solver converges to the optimal objective.} 
\\
\textbf{K = 25} & 25764 & 8810 & 975 & 44.7, 21.8 & 26* - 165 \\
\textbf{K = 30} & 34024 & 11805 & 1175 & 44.7, 21.8 & 165*- TO \\
T = 100 & 29214 & 7215 & 2959 & 44.7, 23 & 62-95* \\

\hline
\multicolumn{6}{|c|}{$\lgSpec_2$} \\
\hline
%\multirow{2}{*}{$\lgSpec_2$} 
% & PWL & 25 & 49581 & 16636 & 1973 & L = 80 $\theta$ = 17.73 & 29* \\
\textbf{K = 25} & 49677 & 16636 & 1973 & 71.4, 17.7 & 38* \\
\textbf{K = 27} & 55371 & 18646 & 2187 & 70, 17.7 & 160* - 195  \\
T = 300 & 192532 & 48275 & 16487 & 70, 17 & 630* - TO \\ 
% & IB & 300 & 69995 (191336) & 28072 (48275) & 2776 (15889) & L = 207.3 $\theta$ = 17 & 65 & 66 & 16\_07\_13\_45\_58 [0 -1] \\ 
% DP1
\hline
\multicolumn{6}{|c|}{$\lgSpec_3$} \\
\hline
%\multirow{4}{*}{$\lgSpec_3$} 
\textbf{K = 23} & 18498 & 6394 & 648 & 75, 0.2 & 6* \\
\textbf{K = 25} & 21209 & 7383 & 706 & 76, 9.7 & 27* \\
\textbf{K = 30} & 28739 & 10153 & 851 & 76, 9.7 & 149* - TO  \\
T = 100 & 21874 & 5537 & 2358 & 76, 10 & 78* - TO \\
\hline
% \multirow{2}{*}{DP1-L} 
% & PWL & 27 & cstr (-) & bin (-) & cont (-) & obj & grb & ym & ... \\
% & DT & 200 & cstr (-) & bin (-) & cont (-) & obj & grb & ym & ... \\
% DP 2
%\hline
\multicolumn{6}{|c|}{$\lgSpec_4$} \\
\hline
%\multirow{2}{*}{$\lgSpec_4$} 
\textbf{K = 35} & 39337 & 11855 & 2090 & 152, 10 & 251* - 305 \\
\textbf{K = 40} & 46577 & 14085 & 2395 & 143, 14.2 & 904* - TO \\
T = 200 & 358929 & 111986 & 8566 & - & TO \\
\hline
\end{tabular}
\caption{Numerical results and the information of the constructed \ac{MILP} between two methods using \ac{PWL} signal and \ac{IB} signal. Our method uses \ac{PWL} signal denoted by the bold letter \textbf{K}, i.e., the number of waypoints. IB method is written in plain text with T denoting the planning horizon. The abbreviations of the \ac{MILP} information from left to right are the number of linear constraints (\# Cstr), binary variables (\# Bin), and continuous variables (\# Cont) respectively. The objective $(L, \theta_+)$ logs the optimized path length, and the right time robustness. The last column logs the solving time of Gurobi in seconds. The number with the symbol $*$ denotes the time that the solver converges to the optimal solution, while the number behind the hyphen (if exists) is the time that the solver needs to terminate the program. ``TO" means time-out, which was set to 1000 seconds to terminate the program.}
\label{tab:bm}
\end{center}
\end{table}

%We briefly summarize that using \ac{PWL} signal offers a more efficient \ac{MILP} encoding compared to IB methods in terms of fewer binary and continuous variables, especially for long-time horizon planning problems. Besides, it is advantageous for planning problems that can be represented through a few numbers of waypoints. Further analysis is required for the solving time of the constructed \ac{MILP}.
We briefly summarize that our method is \emph{sound} and the time-robust \ac{MILP} encoding with \ac{PWL} offers a complexity that is invariant to the planning horizon, which is especially advantageous for problems that can be represented through a few numbers of waypoints, i.e.,  $K^2 \ll T$, but not limited to the cases when $K^2 \approx T$ or $T \ll K^2$ as shown above. 

%3) Further analysis is required for the solving time of the constructed \ac{MILP}.




==> sections/introduction.tex <==
\section{Introduction \& Literature Review} 
%Modern \ac{CPS} offers various potentials to revolutionize a wide range of applications, such as mobility-on-demand, coverage control, rescue operations, smart transportation, and precision agriculture . 
%To formally handle the significant design challenges of the above safety-critical systems, it is essential to have an expressive and reliable mechanism that can capture the complexities.
\emph{Formal Methods} are powerful techniques that utilize logical and reasoning languages with rigorously defined syntax and semantics to express domain expertise unambiguously from natural languages. 
%Such characteristics play a major role in capturing system's complexity, supporting system's design and veficiation.
%support system developments, from requirements analysis to verification. Such methods allow us to , thus playing an essential role in designing and monitoring complex safety-critical systems.  
{One branch of Logic that has been extensively researched and widely used for formal verification is \ac{TL}, an expressive language capable of reasoning logical statements with respect to \emph{time} \cite{Baier2008}}, e.g., a spatial-temporal mission specification ``robot $1$ is \emph{eventually} inside region $A$ and stay there for $5$ time units" can be captured unambiguously with \ac{TL} formulas. Moreover, using \ac{TL} also allows synthesizing robots' trajectories that meet the expected spatial-temporal behaviors with automated algorithms, which is known as the \emph{formal synthesis} problem. 
Recent research focuses on synthesis algorithms using \acrfull{STL} and simultaneously offering \emph{robustness}. \ac{STL} is a sub-branch of \ac{TL} supporting {continuous-time} signals over the reals and quantitative semantics  \cite{Maler2004MonitoringTP}, which allows evaluating the \emph{robustness}, i.e., \emph{degree of satisfaction}, of a signal with respect to a specification. In other words, one may identify ``how much" the system satisfies the requirement, which is essential for automated mission design and synthesis algorithms to encounter possible uncertainties in practice. 

\ac{STL} offers two quantitative semantics: \emph{space} and \emph{time} robustness. Space robustness indicates the spatial margin of a signal regarding specified thresholds, e.g., the \emph{safety-distance} between a trajectory and an obstacle. Formal \ac{STL} synthesis with space robustness is well-studied \cite{Raman2015ReactiveSF, Pang2017Smooth, Lindemann2019ControlBF}. On the other hand, less attention was put on {time robustness}. With time robustness, we can evaluate the performance quantitatively regarding time, e.g., ``the requirement is satisfied with \emph{large time-margin}, or just \emph{in-time}". Such a property is essential as it is hard in practice to assign fixed-time missions, or robots always encounter ubiquitous delays, early starts, or when they have to handle disturbances during executions reactively.
The work \cite{Donze2010RSTL} first defined time-robustness for STL formulas. Afterward, \cite{akazaki2015time, rodionova2021timerobust, Rodionova2022TRTL} further investigated in the context of monitoring and control synthesis. In \cite{rodionova2021timerobust, Rodionova2022TRTL}, the authors proposed a novel strategy to encode time robustness into linear constraints for discretized signal, which allows time-robust synthesis through \acrfull{MILP}. 
Using \ac{MILP} is one paradigm of formal synthesis with \ac{STL} formulas. The pioneering works by \cite{Karaman2008OptimalCO, Raman2015ReactiveSF} proposed the encoding rules using big-M methods \cite{griva2009linear} to transform space-robust \ac{STL} with linear predicates into linear constraints using mixed binary and continuous variables and construct a \ac{MILP}. In this manner, an \ac{STL} control synthesis problem can be formulated into an \ac{MPC}/ optimization problem. Although \ac{MILP}-based approaches are straightforward, {they do not scale well due to the complexity of the constructed \ac{MILP}. In particular, from an \ac{STL} formula, the generated constraints are imposed on \emph{each} discretized trajectory instances, which implies that the \ac{MILP} increases in the number of binary and continuous variables proportionally with the planning horizon. 

Many previous works try to achieve an efficient optimization-based synthesis. The authors in \cite{Pang2017Smooth} propose an approximation method to avoid the computational burden of binary variables in \ac{MILP}, which enables the problem to be solved with Sequential Quadratic Programming.
\cite{Leung2020BackpropagationTS} introduced methods to compute the gradient of the \ac{STL} robustness and allow synthesis with gradient-descent optimization. 
\cite{Lindemann2019ControlBF} suggests constructing time-varying \ac{CBF} from a fragment of \ac{STL} that renders the forward invariant set that satisfies the formula. This approach offers scalability but further attention is required for the general construction of \ac{CBF} functions for various complex specifications. The work \cite{zhang2023modularized} studies a decomposition method to transform long STL formulas into combinations of modularized ones, thus reducing the computational time of \ac{MILP}.} Nevertheless, the above methods are investigated solely for space-robustness. Since the definition of time-robustness involves time-shifting, the above-mentioned methods are not applicable \cite{rodionova2021timerobust}.

{Informally, efficient synthesis from \ac{STL} formula is an open problem. We are motivated to investigate a scalable synthesis method that also offers time-robustness. Our method is directly inspired by the work  \cite{Chuchu2020FGS, Sun20223451} which proposed a novel hierarchical path-planning method using \ac{PWL} signal and their \emph{qualitative} semantics for formal synthesis. 
%a high-level planner to generate \ac{PWL} signal and a low-level tracking controller. 
\ac{PWL} signal considers a trajectory as a sequence of 
waypoints consisting of timestamps and values.  
}
In fact, \cite{Chuchu2020FGS, Sun20223451} shows that various planning problems can be represented by a much less number of waypoints compared to the number of dense-discretized trajectory instances, especially for long-time-horizon planning problems. In this manner, the size of the constructed \ac{MILP} does not scale proportionally with the time horizon but depends solely only on the available number of waypoints. None of these previous works considered time-robustness. We, therefore, propose and investigate the concept of time-robustness for \ac{PWL} signal. The contribution of our study is summarized below
% Our method is strongly related to the previous works by \cite{Chuchu2020FGS, Sun20223451}. The authors in \cite{Chuchu2020FGS} introduce path planning methods using PWL path, which considers a trajectory as sequences of time-stamp waypoints. In this manner, we don't have to impose the constraints on the system at each time-step. Besides, many tasks in practice can be represented through a reasonable \ac{PWL} segment, thus enabling an optimization problem with fewer constraints. \cite{Sun20223451} proposes a qualitative semantics for \ac{PWL} signal to synthesize the desired waypoints.
%Our methods do not impose constraints on each discretized state at each time step of the system as used in \cite{Rodionova2022TRTL}, but instead just introduce constraints on the less number of \ac{PWL} segments that can describe various tasks in practice. \thought{Can you pls help me think of some way to clarify instance-based and interval-based here directly.}

\noindent \textbf{Contributions.} 
\begin{itemize} [leftmargin = *]
    \item \emph{Definition and Quantitative Semantics of Time-Robustness for PWL Signal}: 
    %We formulate the time-robustness STL semantics for \ac{PWL} signal. 
    The notion of time-robust STL was introduced in \cite{Donze2010RSTL} and formally studied in \cite{Rodionova2022TRTL} for instance-based signal. Different from previous works, we review and propose the time-robust STL quantitative semantics for \ac{PWL} signal. We first formally define time robustness for \ac{PWL} signal, then mathematically propose and scrutinize the soundness of the time-interval-based semantics. With our semantics, it is able to express time-robustness directly through the 
    few numbers of waypoints, and also, it allows one to quantitatively evaluate the time-margin of a \ac{PWL} signal with respect to a specification.  
    
    \item \emph{Time-Robust STL Path Planning:} We formulate a novel hierarchical time-robust formal synthesis problem using \ac{PWL} Signal. This problem statement allows us to synthesize the waypoints that not only satisfy a specification but also maximize the time-robustness.
    
    \item \emph{MILP Encoding}: We propose an encoding strategy to transform the studied semantics into a \ac{MILP} problem.
    \item \emph{Experiments}: We implement the synthesis algorithm and use several different mission specifications with different complexity to verify the soundness and our complexity analysis.
\end{itemize}
\textbf{Organization} 
%Section \ref{sec:lr} provides a review of literature studying space-time robust path planning from \ac{STL} formulas. 
Section \ref{sec:prel} introduces the preliminaries including the mathematical notations, qualitative semantics of \ac{STL}, and \ac{PWL} signal. Section \ref{sec:mr} presents the definition and quantitative semantics of time-robust \ac{STL} with \ac{PWL} signal. Section \ref{sec:pf} formally formulates the synthesis problem and introduces a hierarchical planning framework. Section \ref{sec:milp_enc} proposes an encoding strategy to construct a \ac{MILP} for the proposed semantics. Section \ref{sec:bm} provides the numerical experiment results to evaluate the soundness and the performance of our approach. Section \ref{sec:concl} concludes our study.

==> sections/main.tex <==
\section{Time-Robust STL for PWL Signal} \label{sec:mr}
%\def \tr{\text{TR}}
\def \tr{\text{time robustness}}
In this section, we first introduce the notation of time-robust STL according to the previous work \cite{Donze2010RSTL, Rodionova2022TRTL}. Then, we formulate a novel time robustness quantitative STL semantics for \ac{PWL} signal.  
According to \cite{Donze2010RSTL},
{the degree of time-robustness {\tr} is defined as the amount of time $\theta$ that a signal maintains its characteristic with respect to an STL formula. Besides, there are two types of time-robustness: right and left, which respectively distinguish the time margin after and before the specified time instance. In other words, a signal has $\theta^\lgSpec_+$ right-time robustness if it satisfies $\lgSpec$ for \emph{any} preceding time-unit between $[t, t + \theta^\lgSpec_+]$, which allows the synthesized signal to encounter \emph{early start} (left-shifted up to $ \theta^\lgSpec_+$). Meanwhile, left time-robustness is achieved if the signal satisfies $\lgSpec$ for \emph{any} succeeding time-unit between $[t - \theta^\lgSpec_-, t]$, which offers robustness to encounter \emph{delay} (right-shifted up to $ \theta^\lgSpec_-$).       
Let $\trobzj{i}^\lgSpec$  be the right/left time robustness of a PWL signal regarding $\lgSpec$, with ${\bowtie = \{+,-\}}$. We define
%The right/left time robustness indicates the time margin that the signal can be shifted right/left and still maintains its characteristic related to a given specification. This definition was introduced and investigated by the previous works \cite{Donze2010RSTL, RodionovaTRTL} for instance-based signal.
%In our work, we formulate the {\tr} definition for \ac{PWL} signal and its recursive semantics.
\begin{definition}[Time Robustness STL for PWL Signal] \label{def:pwl_tr}
For atomic predicates ${\lgPred}$, the right and left time robustness of a linear segment $z_i$ is defined as
\begin{nalign} \label{eq:pwl_prop_tr_strict}
    &\theta_{+,i}^{{\lgPred}} = \sign(z_i^{\lgPred}) \sum_{j = i+1}^{i + k}(t_{j+1} - t_j), \\ 
    &k = \defkpeq;\\
    &\theta_{-,i}^{{\lgPred}} = \sign(z_i^{\lgPred}) \sum_{j = i-k}^{i-1}(t_{j+1} - t_j), \\
    &k = \defkmeq,
\end{nalign}
when $k = 0$, $\theta_{+,i}^{{\lgPred}} = 0, \theta_{-,i}^{{\lgPred}} = 0$. 

For negation, we use a similar definition but replace $z_i^{\lgPred}$ with $z_i^{\neg \lgPred}$ and $\trobzj{i}^{{\lgPred}}$ with $\trobzj{i}^{{\lgNeg\lgPred}}$. Intuitively, \eqref{eq:pwl_prop_tr_strict} aggregates the time interval of the succeeding/preceding segments $z_{i^\prime}$ as long as they \emph{also} satisfy/violate $\lgPred$ as the segment $z_i$ do, i.e., ${\sign(z_i^{\pi}) = \sign(z^{\pi}_{i^\prime})}$. Specification satisfaction/violation is distinguished by $\sign(z_i^{\pi})$. 
%For negation, since ${z_i^{\lgPred} \neq \lgNeg z_i^{\lgNeg \lgPred}}$ as shown in Remark \ref{rem:pwl_lost_negation}, we use the similar above definition and replace $z_i^{\lgPred}$ with $z_i^{\neg\pi^\mu}$. 
For logical and temporal operators in the recursive syntax \eqref{eq:stl_syntax}, we apply the following semantics 
\begin{align}
    \trobzj{i}^{\lgSpec_1 \lgAnd \lgSpec_2} &= \trobzj{i}^{\lgSpec_1} \infmum \trobzj{i}^{\lgSpec_2}; ~\trobzj{i}^{\lgSpec_1 \lgOr \lgSpec_2} = \trobzj{i}^{\lgSpec_1} \supmum \trobzj{i}^{\lgSpec_2}. && \label{eq:log_time_rob_strict}\\ 
    % alws
    \trobzj{i}^{\stlAlways{a,b}\phi} &= \binfmum_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \label{eq:alws_time_rob_strict} \\ 
    \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_i + a, t_{i+1} + b]  \neq \varnothing\right\}. \notag\\
    % evtll
    \trobzj{i}^{\stlEvtll{a,b}\phi} &= \bsupmum_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \label{eq:evtll_time_rob_strict}\\ %- (t_{i+1} + a - t_{j})
    \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_{i+1} + a, t_i + b] \neq \varnothing\right\}, \notag\\
t_{i+1} + a &\geq t_i + b. \notag\\ 
    % until
     \trobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \bsupmum_{j \in \set{J}^\intersect} \left( \trobzj{j}^{\phi_2} \infmum \binfmum_{l \in \set{L}_j^\intersect}\trobzj{l}^{\phi_1} \right), \label{eq:until_time_rob} \\
    \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing\right\}, \notag\\ 
    \set{L}^\intersect_j &= \left\{l \in \nSet{N}_j | [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing\right\}, \notag\\
    t_{i+1} + a &\geq t_i + b. \notag
\end{align}

% The logical operators \emph{conjunction} and \emph{disjunction}
% can be applied similarly as shown in Definition \ref{def:quanti_tr}, i.e.,
% \begin{nalign} \label{eq:log_time_rob_strict}
%     \trobzj{i}^{\lgSpec_1 \lgAnd \lgSpec_2} &= \trobzj{i}^{\lgSpec_1} \infmum \trobzj{i}^{\lgSpec_2}; ~\trobzj{i}^{\lgSpec_1 \lgOr \lgSpec_2} = \trobzj{i}^{\lgSpec_1} \supmum \trobzj{i}^{\lgSpec_2} &&    
% \end{nalign}
% \hrzline{0.5}
% \begin{nalign} \label{eq:alws_time_rob_strict}
% \trobzj{i}^{\stlAlways{a,b}\phi} &= \binfmum_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \\
% \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_i + a, t_{i+1} + b]  \neq \varnothing\right\}.
% \end{nalign}
% \hrzline{0.5}
% \begin{nalign} \label{eq:evtll_time_rob_strict}
% \trobzj{i}^{\stlEvtll{a,b}\phi} &= \bsupmum_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \\ 
% \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_{i+1} + a, t_i + b] \neq \varnothing\right\},\\
% t_{i+1} + a &\geq t_i + b.
% \end{nalign}
% \hrzline{0.5}
% \begin{nalign} \label{eq:until_time_rob}
%  \trobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \bsupmum_{j \in \set{J}^\intersect} \left( \trobzj{j}^{\phi_2} \infmum \binfmum_{l \in \set{L}_j^\intersect}\trobzj{l}^{\phi_1} \right), \\
% \set{J}^\intersect &= \left\{j \in \nSet{N}_K | [t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing\right\},\\ 
% \set{L}^\intersect_j &= \left\{l \in \nSet{N}_j | [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing\right\}, \\
% t_{i+1} + a &\geq t_i + b.
% \end{nalign}
\end{definition}
%The {\tr} of a segment regarding a conjunction (or disjunction) of two STL formulas is the infimum (or supremum) of the components as shown in  \eqref{eq:log_time_rob_strict}. For temporal operators, 
We provide an explanation for \eqref{eq:alws_time_rob_strict} - the ``always" operator, while the other operators can be understood similarly. The {\tr} $\trobzj{i}^{\stlAlways{a,b}\phi}$ is the minimal (infimum operator) {\tr} $\trobzj{j}^{\phi}$ of \emph{any} segments $z_j$ that intersects with the time interval ${[t_i +a, t_{i+1} +b]}$ (involves in the specified temporal behavior). 

The following theorem formulates the \emph{Soundness} property of the proposed semantics. If segment $z_i$ has positive time robustness regards $\lgSpec$, we know that $z_i$ satisfies $\lgSpec$. Inversely, negative time robustness implies  $z_i$ does not satisfy $\lgSpec$. The equality case is inconclusive.
\begin{theorem}[Soundness] \label{theorem:soundness}
    \begin{nalign}
        \trobzj{i}^{\phi} &> 0 \implies z_i^\phi = \lgTrue &&\hequal z_i \lgSatisfy \lgSpec \\ 
        %\hequal (\xi, t_i) \lgSatisfy \phi \\ 
        \trobzj{i}^{\phi} &< 0 \implies z_i^\phi = \lgFalse &&\hequal z_i \not\lgSatisfy \lgSpec %\hequal (\xi, t_i) \not \lgSatisfy \phi
    \end{nalign}
    \begin{proof}
        See Appendix \ref{apx:sec_proof}.
    \end{proof}
\end{theorem}

\section{Problem Formulation} \label{sec:pf}
Given a spatial-temporal specification expressed as \ac{STL} formula, we aim to synthesize robots' trajectories that satisfy the specification and achieve time robustness. Previous works show that direct synthesis from general \ac{STL} formula is not real-time capable \cite{Pant2018FlyByLogic, Zhou_2015_OMP}. Therefore, we use a \emph{hierarchical} planning framework, i.e., a high-level offline planner synthesizes the reference \ac{PWL} signal (sequence of timestamped waypoints)  that meets a given requirement, and a low-level tracking controller. {Such a control framework is widely used for various autonomous systems. Here, we investigate a path planning problem for quadrotors with differential flatness property using motion primitives \cite{Mueller2015ACEMP, Pant2018FlyByLogic}.} Furthermore, the synthesized signal must consider the feasibility constraints of dynamical systems, e.g., bounded velocity. To ensure the synthesized waypoints satisfy the specification $\lgSpec$ and achieve {\tr}, we formulate an optimization problem for the high-level planner that captures $\lgSpec$ through a set of constraints. Since the expected temporal behavior can be expressed with the time reference $t_0 = 0$, $\lgSpec$ can be expressed with the recursive \ac{STL} syntax. Consequently, we obtain $\trobzj{0}^\lgSpec$ that indicates the {\tr} of a \ac{PWL} path $\xi_{z_0}$ with respect to $\lgSpec$. Formally, we define the time-robust synthesis problem below 
\begin{problem}[Time Robustness STL Planning] \label{prob:opti} Given an STL specification $\lgSpec$, find a sequence of $K-1$ linear segments ${\xi_{z_0} = \{z_{0}, z_{1}, \cdots, z_{K-2}\}}$ that satisfy $\lgSpec$, and maximizes the {\tr} $\trobzj{0}^\lgSpec$.
\begin{align*}
    \max_{\xi_{z_0}} ~& -J(\xi_{z_0}) + \lambda \trobzj{0}^\lgSpec\\
    \text{s.t. } &\trobzj{0}^\lgSpec \geq \theta^* > 0\\ 
     & |v(t)| \leq v_b, 
\end{align*}
where the strict positive $\theta^*$ is the {{\tr} threshold}, $v_b$ is the positive bounded velocity. The objective function $J(\xi_{z_0})$ expresses the desired path properties, e.g., minimal path length, or the shortest make-span. The time robustness is maximized through the term $\trobzj{0}^\lgSpec$. The positive scalar $\lambda >0$ is used to control the objective.
\end{problem}
\begin{remark} \label{rm:assumption}
We assume that the solution of the synthesis problem \emph{exists}. Theorem \ref{theorem:soundness} guarantees that a feasible solution of Problem \ref{prob:opti} satisfies $\lgSpec$ because $\trobzj{0}^\lgSpec$ is strictly positive.    
\end{remark}
\begin{remark} \label{rm:pwl_vs_ib}
Our methods depend on parameter $K$ which is the number of \emph{waypoints} used to represent a trajectory. $K$ has the following impacts
\begin{itemize} [leftmargin = *]
    \item \emph{Complexity}: Let the planning horizons be $T$. We observe that our formulation does not depend on $T$. Indeed, the usage of waypoints allows us to consider $T$ by simply requiring the timestamp of the last waypoint to be ${t_{K-1} = T}$, meanwhile, we are able to represent a signal that is \emph{invariant} to the planning horizon $T$. This property is the advantage of \ac{PWL} signal over instance-based signal when we construct the optimization model, especially for problems with long planning horizons. We offer a more comprehensive complexity analysis in the next section.
    \item \emph{Feasibility}: It is obvious that the trajectory must have sufficient waypoints, thus $K$ can not be chosen arbitrarily. To find the baseline of $K$, one might increase $K$ incrementally until a feasible solution exists (note that we assume Problem \ref{prob:opti} is solvable in Remark \ref{rm:assumption}).
    \item \emph{Solution Quality}: The objective function also depends on $K$ since this parameter decides the solution space of the problem. For instance, with large $K$, more waypoints are available and may offer a better solution. However, the \ac{MILP} complexity will also increase.     
\end{itemize}
%\critical{The complexity also increase with the parameter K. We offer a more comprehensive analysis of the complexity and its dependance on K in section x.} \ac{PWL} signals ($\xi_{z_0}$) are different from the instance-based discretized signal ($\xi$): 1) The timestamps of the waypoints in $\xi_{z_0}$ are unspecified, while we implicitly predefine them for each discretized instance $\xi$ through the fixed time-step; 2) Let the final time-instance be $T$. The number of instances of $\xi$ grows as $T$ increases, while \ac{PWL} signal may use the same number of waypoints and set the timestamp of the last waypoint to be $T$. %Figure \ref{fig:dt_vs_ts} illustrates the differences.     
\end{remark}

\section{\acrfull{MILP}} \label{sec:milp_enc}
To our knowledge, Problem \ref{prob:opti} can not be solved analytically due to the logical operators in a general $\lgSpec$. Therefore, we propose an encoding strategy to transform it into a \ac{MILP}. Considering the timestamps and the spatial locations as optimization variables, the encoding uses additional binary and continuous variables to construct \emph{linear} constraints that correspond to $\trobzj{0}^\lgSpec$. This approach is commonly used \cite{Karaman2008OptimalCO, Raman2015ReactiveSF, Zhou_2015_OMP, Rodionova2022TRTL}. We first introduce the general big-M methods that encode the necessary operators. A detailed explanation of the encoding can be found in \cite{Karaman2008OptimalCO, Raman2015ReactiveSF}. Afterward, we adapt the novel idea of \cite{Rodionova2022TRTL} to encode time-robustness for atomic predicates with \ac{PWL} signal. Our contribution is the encoding for the proposed quantitative semantics.
%In this section, we first introduce the general big-M methods encoding from previous works to construct \emph{linear constraints} for the necessary operators throughout this work, including predicates, logical operators (conjunction/disjunction), infimum/supremum, and multiplication of binary and continuous variables. Afterward, we introduce the {\tr} for predicates inspired by \cite{Rodionova2022TRTL}. Our contribution is the encoding strategy of the proposed {\tr} quantitative semantic of the temporal operators for \ac{PWL} signal.  
\subsection{General \ac{MILP} Encoding} \label{sec:general_MILP}
\begin{itemize} [leftmargin=*]
    \item Linear predicate: each linear predicate is represented through a linear function $\mu(.)$. We use linear predicates to indicate whether \emph{a point} lies in the inside/outside face of an edge of a convex polygon $\mathcal{P}$ (see \eqref{eq:zpi_sdp}). For instance, let 
    ${\mu(p_i) = \frac{h^j - A^jp_i}{\norm{A^j}_2} \geq \epsilon}$ be a linear function. If $\mu(p_i) \geq 0$, $p_i$ lies \emph{inside} the edge $(A^j, h^j)$ of $\mathcal{P}$ with $\epsilon$ space margin. We can capture $\mu(p_i) \geq 0$  through a binary variable $b^{\mu}$ as
    \begin{flalign} \label{eq:milp_lin_pred}
    -M(1 - b^{\mu}) &\leq {\mu}(p_i) \leq Mb^{\mu} - m_\epsilon,
    \end{flalign}
    where $M, m_\epsilon$ are sufficiently large and small positive numbers respectively. If $b^{\mu} = 1$, ${\mu}(p_i) \geq 0$, else ${\mu}(p_i) < 0$. For the case ``\emph{outside} $(A^j, h^j)$ by $\epsilon$ space margin", we apply the same encoding method with ${\mu(p_i) = \frac{A^jp_i - h^j}{\norm{A^j}_2} \geq \epsilon}$. 

    \item Conjunction of $m$ binary variables, i.e., $b = \bigwedge_{i = 1}^m b_i$, is encoded through the following constraints ${b \leq b_i, \forall i \in \nSet{N}_m}$ \text{ and } ${b \leq \sum_{i = 1}^m b_i - (m-1).}$
    % \begin{nalign} \label{eq:conj_disj}
    % b \leq b_i, \forall i \in \{1 \cdots m\} \text{ and } b \leq \sum_{i = 1}^m b_i - (m-1).
    % \end{nalign}

    \item Disjunction of $m$ binary variables, i.e., $b = \bigvee_{i = 1}^m z_i$ is guaranteed with ${b \geq b_i, \forall i \in \nSet{N}_m}$ \text{ and } ${b \leq \sum_{i = 1}^m b_i.}$
    % \begin{nalign} \label{eq:disj}
    %     b \geq b_i, \forall i \in \{1 \cdots m\}  \text{ and } b \leq \sum_{i = 1}^m b_i.
    % \end{nalign}
    
    \item The infimum of $m$ continuous variables, i.e., $\binfmum_{i = 1}^m \theta_i$, is encoded through a continuous variables $\theta$ by introducing $m$ binary variables $\{b_1, \cdots, b_m\}$ and impose the following linear constraints
% \begin{nalign} \label{eq:min_enc}
%     \phi &= \bigwedge_{j = 1}^N \phi_i: \trob^{\phi} = \min ( \trob^{\phi_1},  \trob^{\phi_2}, \cdots  \trob^{\phi_N})\\
%     &\trob^{\phi_j} - (1 - b_j)M \leq \trob^{\phi} \leq \trob^{\phi_j} + (1 - b_j)M, \\ 
%     & ~\trob^{\phi} \leq \trob^{\phi_j} ~ \forall j \in \{1 \cdots N\}, ~\sum_{i = 1}^{N} b_j = 1
% \end{nalign}
% \begin{nalign} \label{eq:max_enc}
%     \phi &= \bigvee_{j = 1}^N \phi_i: \trob^{\phi} = \max (\trob^{\phi_1}, \trob^{\phi_2}, \cdots  
%     \trob^{\phi_N}) \\ 
%     &\trob^{\phi_j} - (1 - b_j)M \leq \trob^{\phi} \leq \trob^{\phi_j} + (1 - b_j)M, \\
%     & ~ \trob^{\phi} \geq \trob^{\phi_j}, ~ \forall j \in \{1 \cdots N\}, ~\sum_{i = 1}^{N} b_j = 1
% \end{nalign} 
    \begin{subequations} \label{eq:inf_sup}  
    \begin{align}        
        & \theta_i - (1 - b_i)M \leq \theta \leq \theta_i, \forall i \in \nSet{N}_m, \label{eq:inf_sup-a} \\ 
        &\sum_{i = 1}^{m} b_i = 1. \label{eq:inf_sup-b}
        \end{align}
    \end{subequations}
Equation \eqref{eq:inf_sup-a} ensures that $\theta$ is smaller than other variables and equal to any $\theta_i$ if and only if $b_i = 1$. Equation \eqref{eq:inf_sup-b} ensures that the infimum of the set exists. For supremum, we use the similar above encoding constraints, but replace \eqref{eq:inf_sup-a} with ${\theta_i \leq \theta \leq \theta_i + (1 - b_i)M}$.

\item {Multiplication  $y = xb, x \in \nSet{R}, b \in \nSet{B}$:} we impose
\begin{nalign} \label{eq:multi_xb}
  -Mb \leq y \leq Mb,~ x - M(1 - b) \leq y \leq x + M(1 - b),  
\end{nalign}
with positive $M$ is the sufficient large upper bound of $x$.
\end{itemize}


\subsection{{Time Robustness} Encoding for \ac{PWL} signal} \label{sec:tre}
Throughout this section, we use the right-time robustness to explain the encoding that corresponds to the definition of {\tr} in Definition \ref{def:pwl_tr}. A similar strategy can be applied for the left time robustness. We first introduce the time robustness encoding for the atomic predicates, and then for the temporal operators.
\begin{itemize} [leftmargin=*]
 \item Let $\rtrobzj{i}^{{\lgPred}}$ be the right {\tr} of segment $z_i$ regarding atomic predicate $\lgPred$, we adapt the ``counting" encoding concept proposed by the authors in \cite{Rodionova2022TRTL} to generate linear constraints such that $\rtrobzj{i}^{{\lgPred}}$ correspond to the right {\tr} in \eqref{eq:pwl_prop_tr_strict}. To this end, we introduce two \emph{continuous} \emph{time-aggregating} variables $\Delta t^1_i$ and $\Delta t^0_i$  for \emph{each} segment and encode $\rtrobzj{i}^{{\lgPred}}$ as follows 
\begin{align}
    \Delta t^1_i &= (\Delta t^1_{i+1} + \delta t_i)z_i^{\lgPred},
    \Delta t^0_i = (\Delta t^0_{i+1} - \delta t_i)(1 - z_i^{\lgPred})  \label{eq:t_aggre}\\
    \rtrobzj{i}^{{\lgPred}} &= \Delta t^1_i  + \Delta t^0_i + \left(- z_i^{\lgPred}\delta_i + (1 - z_i^{\lgPred})\delta_i \right) \label{eq:tr_raw}\\ 
    &= z_i^{\lgPred}\Delta t^1_{i+1} + (1 - z_i^{\lgPred})\Delta t^0_{i+1} \label{eq:right_time_rob},
\end{align}
with ${\delta t_i = t_{i+1} - t_i}$, ${\Delta t^1_{K-1} = \Delta t^0_{K-1} = 0}$.

According to \eqref{eq:pwl_prop_tr_strict}, the constraints depend on $z_i^\lgPred$, i.e., the qualitative value of segment $z_i$ with respect to the atomic predicate $\lgPred$. As defined in \eqref{eq:zpi_sdp}, $z_i^\lgPred$ indicates whether \emph{a segment} $z_i$ lies inside $\mathcal{P}$, which is constructed through conjunction and disjunction of linear predicates according to \eqref{eq:zpi_sdp}. Therefore, we apply the encoding techniques in Section \ref{sec:general_MILP} to obtain the constraints for $z_i^\lgPred$.

Next, we use $\Delta t^1_i$ and $\Delta t^0_i$ distinguish the sign operator in \eqref{eq:pwl_prop_tr_strict}, i.e., $\sign z_i^\lgPred$. In particular, \eqref{eq:t_aggre} implies that $\Delta t^1_i$ aggregates the time interval of the successive segments $z_{i+1}$ if ${z^\lgPred_{i+1} = z^\lgPred_{i} = 1}$, while  $\Delta t^0_i$ aggregate the negative time interval, i.e.,  $-\delta t_i$ if $z^\lgPred_{i+1} = z^\lgPred_{i} = 0$. Moreover, since \eqref{eq:t_aggre} is recursive, the aggregation continues until $z_{i+1} \neq z_{i}$. This corresponds to the $\sum$ operator used in \eqref{eq:pwl_prop_tr_strict}. 

Finally, since these variables are disjunctive, i.e., ${\Delta t^1_i \neq 0 \implies \Delta t^0_i = 0}$ and vice versa \cite{Rodionova2022TRTL}, they can be combined into $\Delta t^1_i  + \Delta t^0_i$ as shown in \eqref{eq:tr_raw}. The last summand in \eqref{eq:tr_raw} is explained by the fact that the {\tr} defined in \eqref{eq:pwl_prop_tr_strict} does not contain the time interval $\delta_i$ of the current segment $z_i$, so we have to subtract or add $\delta_i$ according to the sign of $z_i$. The encoding for negation $\lgNeg \lgPred$ is performed similarly by replacing $z^\lgPred_{i}$ and $\rtrobzj{i}^{{\lgPred}}$  with $z^{\lgNeg\lgPred}_{i}$ and $\rtrobzj{i}^{{\lgNeg\lgPred}}$. 

Furthermore, we emphasize that \eqref{eq:t_aggre} and  \eqref{eq:right_time_rob} can be realized with linear constraints by using the encoding for multiplication of binary and continuous variables in \eqref{eq:multi_xb}.

\item For temporal operators, we instruct the encoding for the ``eventually" ($\tlEvtll$), the other operators can be done similarly. Recall the expression from \eqref{eq:evtll_time_rob_strict}, let $\trob^*$ be $\trobzj{i}^{\stlEvtll{a,b}\lgSpec}$, we introduce $K-1$ additional binary variables $\{b_1, \cdots, b_{K-1}\}$ and impose the following constraints
\begin{subequations} 
\begin{flalign}
%& b_{ij}^\intersect \lgEqual [t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i + b] \neq \varnothing, t_{i+1} - t_i \leq b - a, \label{eq:timeintrs_evtll_tr}\\
& b_{ij}^\intersect \lgEqual (t_{i}+b - t_j \geq \epsilon_t) \lgAnd (t_{j+1} - (t_{i+1} +a) \geq \epsilon_t) \notag \\
& ~~~~~~ \lgAnd \left(t_{i+1} - t_i \leq b - a\right), \forall j \in \nSet{N}_K; \label{eq:timeintrs_evtll_tr}\\
& \trobzj{j}^\lgSpec - (1- b_{ij}^\intersect)M \leq \trob^*, \forall j \in \nSet{N}_K; \label{eq:geq_evtll_tr} \\
& \trob^* \leq \trobzj{j}^\lgSpec + (1- b_{j})M, \forall j \in \nSet{N}_K; \label{eq:evtll_tr_leq}\\  
& b_{ij}^\intersect \geq b_j, \forall j \in \nSet{N}_K; \sum_{j = 1}^K b_j = 1. \label{eq:supremum_exists}
\end{flalign}
\end{subequations} 
First, in \eqref{eq:timeintrs_evtll_tr}, the binary variable $b^\intersect_{ij}$ with $\epsilon_t \in \nSet{R}_{\geq 0}$ indicates whether two time-intervals $[t_j, t_{j+1}]$ and ${[t_{i+1} +a, t_{i} +b]}$ intersects. If $b^\intersect_{ij} = \lgTrue$, they intersect, else they don't. Equation \eqref{eq:geq_evtll_tr} implies that $\trob^*$ is greater or equal to the time robustness of \emph{any} segments that intersect with $[t_{i+1} +a, t_i + b]$. Meanwhile, \eqref{eq:evtll_tr_leq} guarantees that $\trob^*$ is bounded by $\trobzj{j}^\lgSpec$ whenever $b_{j} = 1$. Finally, \eqref{eq:supremum_exists} ensures that the supremum belongs to the given set that intersects, i.e, $b_j = 1 \implies b_{ij}^\intersect = 1$. Besides, $\sum_{j = 1}^K b_j = 1$ ensures that the supremum exists.
\end{itemize}


\subsection{Complexity Analysis} \label{sec:complex_ana}
We analyze the encoding complexity for a \ac{PWL} signal $\xi_{z_0}$ with $K$ segments.
Atomic predicates (AP) (or negations) are constructed through the set of $|AP|$ linear predicates, thus we need $\bigO(|AP|K)$ binary variables for $\xi_{z_0}$. Time robustness for AP requires $\bigO(1)$ additional continuous variables for each segment as shown in \eqref{eq:t_aggre}, thus $\bigO(K)$ for $\xi_{z_0}$. For temporal operators, we need additional variables to encode the time-intersection and infimum/supremum. Each segment requires $\bigO(K)$ additional binary and $\bigO(1)$ continuous variables, which respectively results in $\bigO(K^2)$ and $\bigO(K)$ for $\xi_{z_0}$. Let the formula $\lgSpec$ has $|\lgSpec|$ operators, the generalized number of binary and continuous variables of \ac{MILP} is $\bigO(|\lgSpec|K^2)$ and $\bigO(|\lgSpec|K)$ respectively \footnote{For a formula with \emph{one single temporal operator}, e.g., $\stlEvtll{I} {\lgPred}$, $\stlAlways{I} {\lgPred}$, we just impose constraints on the first segment, thus only requiring $\bigO(|AP|K)$ binary variables instead of $\bigO(|AP|K + |\lgSpec|K^2)$}. 

Compared to the instance-based signal with $T$ instances, the complexity shown in \cite{Rodionova2022TRTL} is {$\bigO(|AP|T)$} binary and $\bigO(|\lgSpec|T)$ continuous variables. Although using \ac{PWL} signal has the quadratic term $K^2$ complexity, various path-planning problems can be represented in practice with $K^2 \ll T$. For this reason, we informally define \emph{long horizon} planning problem as a synthesis problem with the number of waypoints satisfying $K^2 \ll T$. Moreover, the analysis confirms Remark \ref{rm:pwl_vs_ib} that the encoding with \ac{PWL} signal \emph{does not depend on $T$}, which shows the advantage of \ac{PWL} signal long-time horizon planning problems.
% \critical{To be discussed.
% \begin{itemize}
%     \item $\bigO(|\lgSpec|K)$ if $|\lgSpec| = 1$.
%     \item $|\lgSpec|K << |\lgSpec|T$
%     \item $|\lgSpec|K^2 \approx ? |\lgSpec|T$
%     \item It should be $\bigO(|\lgSpec|T^2)$ for the "Until" operator, why no previous works mention it?
% \end{itemize}
% }

% \begin{remark}
%     We use $\bigO(K^2)$ binary variables and $\bigO(K)$ continuous variables to encode the "until" operators. \thought{The encoding is sound, but I will double-check it later if we can further reduce the complexity.}
% \end{remark}

\subsection{Algorithm Overview}
We formally summarize our approach through the following algorithms. The synthesis first initializes the \ac{PWL} signal ${\xi_{z_0}}$ as optimization variables. The \ac{STL} encoding is performed modularized for each region $\mathcal{P}$ and recursive for temporal operators (Algorithm \ref{alg:sr_ra}). Afterward, we combine the linear constraints obtained from the encoding of \emph{every} regions, and additionally consider dynamical constraints to construct a complete \ac{MILP} (Algorithm \ref{alg:all_in} - see Appendix \ref{apx:algo2} \critical{If we don't have enough space for Apdx III, we have to summarize Algo 2 in words}).   
\def \cstrSetFinal{$\mathcal{X}_\lgSpec$}
\def \cstrSet{$\mathcal{X}$}
\begin{algorithm}[H] 
\caption{Single Region Reach-Avoid Specification}
\label{alg:sr_ra}
\begin{algorithmic}[1]
\Require{Region $\mathcal{P}$, STL Formula $\lgSpec$ for $\mathcal{P}$, number of waypoints $K$, variables of \ac{PWL} Trajectory ${\xi_{z_0}}$ 
%${\xi_{z_0} = \{z_{0}, z_{1}, \cdots, z_{K-2}\}}$ 
from Definition \ref{def:pwl_traj}} 
\Ensure{Set of linear constraints \cstrSetFinal}
\State \cstrSetFinal $\gets$ \{\}
\State $A \in \nSet{R}^{m \times 2} , b \in \nSet{R}^{m}$ $\gets$ Convex Approximation of $\mathcal{P}$ 
\For{$j \gets 1$ to $m$}                    
    \For{$z_i^\lgPred \gets z_0^\lgPred$ to $z_{K-1}^\lgPred$}                    
        \State $z_i^\lgPred$, \cstrSet $\gets$ \eqref{eq:zpi_sdp}, $A^j, b^j$
        \State \cstrSetFinal $\gets$ \{\cstrSetFinal, \cstrSet\} 
    \EndFor 
\EndFor

\For{$z_i^\lgPred \gets z_0^\lgPred$ to $z_{K-1}^\lgPred$}   
    \State $\trobzj{i}^\lgPred$, \cstrSet  $\gets$ $z_i^\lgPred$, \eqref{eq:right_time_rob}
    \State \cstrSetFinal $\gets$ \{\cstrSetFinal, \cstrSet\}
\EndFor

\For{temporal operators in $\lgSpec$ (backward, recursive)}      \State $\trobzj{i}^\lgSpec$, \cstrSet $\gets$ Applies Section \ref{sec:milp_enc} for $\trobzj{i}^\lgPred$
    \State \cstrSetFinal $\gets$ \{\cstrSetFinal, \cstrSet\}
\EndFor
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[H] 
% \caption{Time-Robust Synthesis with MILP}
% \label{alg:all_in}
% \begin{algorithmic}[1]
% \Require{STL Formula $\lgSpec$, number of waypoints $K$, maximal velocity $v_b > 0$, makespan $T > 0$} 
% \Ensure{${\xi_{z_0}}$}
%     \Statex{// Setup}
%     \State Initialize decision variables ${\xi_{z_0}}$
%     \State \cstrSetFinal $\gets$ \{\}
    
%     \Statex{// STL constraints}
%     \For{ each region $\mathcal{P}$ in $\lgSpec$}   
%     \State \cstrSet $\gets$ Algorithm \ref{alg:sr_ra}($\mathcal{P}$, $\lgSpec$, $K$, $\xi_{z_0}$) 
%     \State \cstrSetFinal $\gets$ \{\cstrSetFinal, \cstrSet\}
%     \EndFor

%     \Statex{// Dynamic constraints for the waypoints}
%     \State \cstrSetFinal $\gets$ \{\cstrSetFinal, $t_0 = 0, t_{K-1} = T$\}
%     \Statex    
%     {// Loop over each pair of waypoints $\tuple{t_i, p_i, t_{i+1}, p_{i+1}}$}
%     \For{i $\gets$ 0 to $K-1$}   
%     \State \cstrSetFinal $\gets$ \{\cstrSetFinal, $t_{i+1} \geq t_{i}, |p_{i+1} - p_{i}| \leq v_b (t_{i+1} - t_{i})$\}
%     \EndFor

%     \State{// MILP Synthesis}
%     \State ${\xi_{z_0}}$ $\gets$ GUROBI(\cstrSetFinal, $J({\xi_{z_0}})$)    
% \end{algorithmic}
% \end{algorithm}

% The algorithm constructs a \ac{MILP} from the STL formula
% \begin{itemize}
%     \item Input: time horizon, velocity max, STL formula
%     \item We initialize a sequence of $K$ waypoints 
%     \[\{(x_1, y_1, t_1) \cdots (x_K, y_K, t_K)\}\]
%     \item Impose the feasibility constraints
%     \begin{align*}
%         0 &= t_{1} \leq t_{2} \leq \cdots \leq t_{K} = T_{\max} \\
%         v_b (t_{i+1} - t_i) &\leq x_{i+1} - x{i} \leq v_b (t_{i+1} - t_i) \\
%         v_b (t_{i+1} - t_i) &\leq y_{i+1} - y{i} \leq v_b (t_{i+1} - t_i)
%     \end{align*}
%     \item Impose the linear constraints generated from STL formulas. See section \ref{sec:milp_enc}. 
% \end{itemize}














==> sections/mod_pwl.tex <==
\subsection{Modified Time-Robustness Semantics for PWL Trajectory}
\begin{definition}[Modified Time Robustness Encoding for PWL]
For atomic proposition $\pi$, the right and left time robustness of a trajectory is encoded as
\begin{nalign} \label{eq:pwl_prop_tr}
    \theta_{+,z_i}^{\pi} &= \sign(z_i) \sum_{j = i}^{i + k}(t_{j+1} - t_j), \\ 
    k &= \argmax_{\{0, 1, \cdots, K\}} \forall i^\prime \in \{i+1, \cdots, i+k\}, \sign(z_i) = \sign(z_{i^\prime});\\
    \theta_{-,z_i}^{\pi} &= \sign(z_i) \sum_{j = i-k}^{i}(t_{j+1} - t_j), \\
    k &= \argmax_{\{0, 1, \cdots, K\}} \forall i^\prime \in \{i-k, \cdots, i-1\}, \sign(z_i) = \sign(z_{i^\prime}).
\end{nalign}

\thought{When $k = 0$, $\theta_{+,z_i}^{\pi} = t_{i+1} - t_i, \theta_{-,z_i}^{\pi} = -(t_{i+1} - t_i)$}.

\begin{remark} \label{rem:strict_time_rob}
An interesting aspect that we must consider is the meaning of the "time robustness" of a linear segment regarding a proposition. For instance, if we say that segment $z_i$ holds true for a proposition $\pi$, we imply that $\pi$ is true for any time between $t_i$ and $t_{i+1}$. However, the "time-robustness" (supposed right-time robustness) is different at $t_i$ and $t_{i+1}$, i.e., we know that at $t_i$, the proposition holds for at least the next $t_{i+1} - t_i$, while at $t_{i+1}$, the time-robustness depends on the next segment. \thought{This observation suggests that we have to address the problem using time-interval semantics for STL. In this work, the time-robustness wrt a proposition strictly \emph{includes} the time interval of the segment as defined in \eqref{eq:pwl_prop_tr}. Further constraints are imposed to reflect the degree of time robustness wrt temporal operators.}
\end{remark}

Time robustness is encoded recursively for the temporal operators according to Definition \ref{def:quanti_tr} as follows:
\hrzline{0.5}
\begin{nalign} \label{eq:alws_time_rob}
\rtrobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \rtrobzj{j}^\phi + (t_j - (t_{i+1} +b)), \\
\ltrobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \ltrobzj{j}^\phi - (t_{j+1} - (t_{i} +a)), \\
% \trobzj{i}^{\stlAlways{a,b}\phi} &= \min_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \\
\set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \\ 
{b^\intersect_{ij}} &\lgEqual [t_j, t_{j+1}] \intersect [t_i + a, t_{i+1} + b].
\end{nalign}
%
\hrzline{0.5}
\begin{nalign} \label{eq:evtll_time_rob}
\trobzj{i}^{\stlEvtll{a,b}\phi} &= \max_{j \in \set{J}^\intersect} \trobzj{j}^\phi, \\ %- (t_{i+1} + a - t_{j})
\set{J}^\intersect &= \left\{1 \cdots K | b^\intersect_{ij} = 1\right\}, \\ 
% \critical{b^\intersect_{ij}} &= \left([t_j, t_j+1] \intersect [t_{i+1} + a, t_i + b] \neq \varnothing\right). \\
{b^\intersect_{ij}} &\lgEqual t_j \in [t_{i+1} + a, t_{i} + b].
\end{nalign}
Different from the qualitative semantics \eqref{eqn:pwl_stl}, we consider only segments that lie strictly within the considered interval. 

\hrzline{0.5}
\begin{nalign} \label{eq:until_time_rob}
 \trobzj{i}^{\phi_1\stlUntil{a,b}\phi_2} &= \max_{j \in \set{J}^\intersect}\left( \min \left( \trobzj{j}^{\phi_2}, \min_{l \in \set{L}_j^\intersect}\trobzj{l}^{\phi_1} \right)\right),
 \\
\set{J}^\intersect &= \left\{1 \cdots K | t^\prime \in [t_j, t_{j+1}]\right\}, \set{L}^\intersect_j = \left\{1 \cdots j | t^\prime \in [t_l, t_{l+1}]\right\}, \\
% b^\intersect_{ij} &= (, \\
% b^\intersect_{il} &=  \\
t_{i+1} + a &\leq t^\prime \leq t_i +b.
\end{nalign}
%where $M$ is a sufficiently large positive number.
\end{definition}
%\hrzline{0.5}

\critical{
\begin{theorem}[Soundness] \label{theorem:soundness}
The imposed constraints for $\trob^{\phi}$ ensure that the corresponding trajectory satisfies the requirement.
\begin{nalign}
    \trob^{\phi}(z_i) &> 0 \implies z_i^\phi = ~\lgTrue \hequal (\xi, t_i) \lgSatisfy \phi \\ 
    %\trob^{\phi}(z_i) &< 0 \implies z_i^\phi = ~\lgFalse \hequal (\xi, t_i) \not \lgSatisfy \phi
\end{nalign}
\begin{proof}
    See Appendix \ref{apd:mod_tr}
\end{proof}
\end{theorem}
}

==> sections/preliminaries.tex <==
\section{Preliminaries} \label{sec:prel}

\subsection{Mathematical Notation}
True and False are denoted by $\lgTrue, \lgFalse$ respectively. We use the set ${\nSet{B} = \{\lgFalse, \lgTrue\} = \{0, 1\}}$ to denote both sets of boolean and binary values. The set of natural, integer, and real numbers are $\nSet{N}, \nSet{Z}, \nSet{R}$ respectively. $\nSet{Z}_{\geq 0}, \nSet{R}_{\geq 0}$ are the set of non-negative integers and real numbers. The set of strict positive natural index $\nSet{N}_K$ denotes $\{1, 2, \cdots, K\}$. To represent a signal, $\nSet{X}$ is the signal space, and $\nSet{T}$ expresses the space of time-instance, which is either the time index (integers) for the discretized signal or the time instant (reals).
We use $\infmum$ for infimum and $\supmum$ supremum operators. The assignment operator is $\lgEqual$. The Euclidean norm is written as ${\norm{.}_2}$. The ``equivalence" of expressions is written with $\hequal$. Additionally, we define the sign operator $\sign(.)$ over boolean variables 
\begin{nalign}
    % \sign(x): \nSet{R} \xrightarrow{} \{-1,0,1\} = 
    % \begin{cases}
    %     1 & x \geq 0 \\
    %     %0 & x = 0 \\
    %     -1 & x < 0
    % \end{cases}, \\
    \sign(x): \nSet{B} \xrightarrow{} \{-1,1\} = 
    \begin{cases}
        1 & x = 1 \\
        -1 & x = 0
    \end{cases}.    
\end{nalign}

%\textcolor{blue}{let's make a section called comparison with instance-based and move equations 2 and 5 there.}
\subsection{Signal Temporal Logic (STL)}
We first introduce the notation of signal and \ac{STL} based on the instance-based (or point-wise) semantics which considers a signal as a sequence of states $x_i$ at each discrete time instant $t_i$.
%\begin{definition}[Signal]
% An instance-based signal with a time horizon $T$ is defined as
% \begin{nalign}
%     \xi_{t_0} &= [\xi(t_0), \xi(t_1), \cdots, \xi(t_{T-1})],
% \end{nalign}
Let ${\xi}$ be a discretized signal where $\xi(.): \nSet{T} \xrightarrow{} \nSet{X}$ denotes the signal value at time instant $t_i \in \nSet{T} \subseteq \nSet{Z}_{\geq 0}$ and $\xi(t_i) \in \nSet{X} \subseteq \nSet{R}^d$ for signal with $d$ dimensions. 
%To simplify the notation, we use $\xi$ to indicate a signal if the starting time $t_0$ and the time horizon is not important. 
Moreover, in the context of motion planning for robots, signals represent robots' trajectory, thus we use \emph{signal} and \emph{trajectory} interchangeably.
%\end{definition}
The syntax and semantics of \ac{STL} are defined below 
\begin{definition}[STL Syntax]  \label{def:stl_syntax} 
\begin{align} \label{eq:stl_syntax}
    \lgSpec \lgEqual  {\lgPred} | \lgNeg {\lgPred} | \lgSpec_1 \lgAnd \lgSpec_2 | \lgSpec_1 \lgOr \lgSpec_2 | \tlEvtll_{I} \lgSpec | \tlAlways_{I} \lgSpec | \lgSpec_1\tlUntil_{I}\lgSpec_2,  
\end{align}
% \textcolor{blue}{add a comment that $\stlEvtll{a,b}$ and $\stlAlways{a,b}$ can be derived from the other operators, right?}
where ${\lgPred}$ and ${\lgNeg\lgPred}$ denote an atomic predicate and its negation,
$\lgSpec_1$ and $\lgSpec_2$ are formulas of class $\lgSpec$. {The logical operators are conjunction ($\lgAnd$) and disjunction ($\lgOr$).} Temporal operators are ``Eventually" ($\tlEvtll$), ``Always" ($\tlAlways$) and ``Until" ($\tlUntil$) with the subscript $I$ denotes the time interval ${[a,b], 0 \leq a \leq b}$. Similar to \cite{Sun20223451}, we use \emph{Negation Normal Form} syntax, i.e., negation is applied only to atomic predicates ${\lgPred}$. It is not restrictive because we can express any \ac{STL} formula using this syntax \cite{Sun20223451}. 
% Besides, the relation between these operators are ${\stlEvtll{a,b}\lgSpec \hequal \lgTrue \stlUntil{a,b} \lgSpec}$, ${\stlAlways{a,b}\lgSpec \hequal \neg \stlEvtll{a,b} \neg \lgSpec}$.     
\end{definition} 
{We assume that the atomic predicates can be represented by linear function}. Let ${\mu(.): \nSet{X} \xrightarrow{} \nSet{R}}$ be a real value linear function that maps a signal instance to a real value. Such function represents an atomic predicate ${\lgPred}$ through the relationship ${{\lgPred} \lgEqual \mu(\xi(t)) \geq 0}$, i.e., ${\lgPred}$ holds \emph{true} if and only if $\mu(\xi(t)) \geq 0$. In the following, we introduce the qualitative semantics of STL which define when a signal satisfies a formula $\lgSpec$ at time point $t$. In particular, we have $(\xi, t) \lgSatisfy \lgSpec$ means $\xi$ satisfies $\lgSpec$ at $t$, and 
$(\xi, t) \not\lgSatisfy \lgSpec$ if $\xi$ does not satisfy $\lgSpec$ at $t$. The semantics are defined \emph{recursively} for each formula in the syntax \eqref{eq:stl_syntax} below
\begin{definition}[Qualitative Semantics of STL formulas%\cite{Maler2004MonitoringTP}
]
\begin{nalign} \label{eqn:qual_stl_semantics}
    (\xi, t) &\lgSatisfy {\lgPred} && \lgIff \mu(\xi(t)) \geq 0\\
    (\xi, t) &\lgSatisfy \tlNot{\lgPred} && \lgIff (\xi, t) \not\lgSatisfy {\lgPred}\\ 
    (\xi, t) &\lgSatisfy \lgSpec_1 \lgAnd \lgSpec_2 && \lgIff (\xi, t) \lgSatisfy \lgSpec_1 \lgAnd (\xi, t) \lgSatisfy \lgSpec_{2} \\ 
    (\xi, t) &\lgSatisfy \lgSpec_1 \lgOr \lgSpec_{2} && \lgIff (\xi, t) \lgSatisfy \lgSpec_1 \lgOr (\xi, t) \lgSatisfy \lgSpec_{2} \\ 
    (\xi, t) &\lgSatisfy \stlEvtll{a,b} \lgSpec && \lgIff \exists {{t^\prime} \in [t+a,t+b]} ~ (\xi, t^\prime) \lgSatisfy \lgSpec \\ 
    (\xi, t) &\lgSatisfy \stlAlways{a,b} \lgSpec && \lgIff \forall {{t^\prime} \in [t+a,t+b]} ~ (\xi, t^\prime) \lgSatisfy \lgSpec \\ 
    (\xi, t) &\lgSatisfy \lgSpec_1 \stlUntil{a,b} \lgSpec_2 && \lgIff \exists t^\prime \in [t + a, t + b], (\xi, t^\prime) \lgSatisfy \lgSpec_{2} \\ 
    & && \lgAnd 
    (\forall t^{\prime \prime} \in [t, t^\prime], (\xi,{t^{\prime\prime}}) \lgSatisfy\lgSpec_1) 
\end{nalign}  
\end{definition}

%Moreover, we also use the notation $\xi_t^\lgSpec$ as a binary variable that indicates whether ${(\xi, t) \lgSatisfy \lgSpec}$. We have the following relationship
% \critical{Rewrite in English with formulas}
% \begin{nalign}
%   \xi_t^\lgSpec & \lgEqual (\xi, t) \lgSatisfy \lgSpec,\\  
%   \xi_t^\lgSpec = \lgTrue &\iff \sign{(\xi_t^\lgSpec)} = 1 \iff (\xi, t) \lgSatisfy \lgSpec, \\
%   \xi_t^\lgSpec = \lgFalse &\iff \sign{(\xi_t^\lgSpec)} = -1 \iff (\xi, t) \not\lgSatisfy \lgSpec. \\
% \end{nalign}

\subsection{\acrfull{PWL} Trajectory}
Instead of using a discretized signal to represent a robot's trajectory, one may use a sequence of timestamped waypoints with the assumption that the path between each pair of waypoints is linearly connected. We define \ac{PWL} signal below
\begin{definition}[Waypoint]
A waypoint is a tuple consisting of a timestamp and the signal value  
\begin{align}
 w = \tuple{t, p}, t \in \nSet{T} \subseteq \nSet{R}_{\geq 0}, p \in \nSet{X} \subseteq \nSet{R}^d.   
\end{align}
\end{definition}
\begin{definition}[Linear Waypoint Segment]
A linear waypoint segment is a pair of a starting and an ending waypoint,
${z}_i = \{w_i, w_{i+1}\} \hequal \{\tuple{t_i, p_i}, \tuple{t_{i+1}, p_{i+1}}\}$ with ${0 \leq t_i \leq t_{i+1}}$. The value of each time instance of a segment can be represented by a linear function ${Z_i(.): \nSet{T} \xrightarrow{} \nSet{X}}$, i.e.,
\begin{nalign}
Z_i(t) & = p_i + \frac{p_{i+1} - p_{i}}{t_{i+1} - t_i}(t - t_i),  t \in [t_i, t_{i+1}]
\end{nalign}
\end{definition}
\begin{definition}[\acrfull{PWL} Trajectory] \label{def:pwl_traj}
A piece-wise linear trajectory from $K$ waypoints is a sequence of $K - 1$ linear waypoint segments
${\xi_{z_0} = \{z_{0}, z_{1}, \cdots, z_{K-2}\}}$. 
\end{definition}

% The following remark clarifies the differences between \ac{PWL} signal ($\xi_{z_0}$) and the instance-based (IB) ($\xi$) signals.
% \begin{remark} ~
%     \begin{itemize}
%         \item For a given planning-time horizon $T$, the number of instances of (IB) signal increases inverse proportionally with the time-step between each instance, while the number of waypoints $K$ of \ac{PWL} signal is predefined and invariant from $T$.
%         \item The number of waypoints $K$ of \ac{PWL} signal is given or predefined according to each planning scenario.
%     \end{itemize}
% \end{remark}


%By this definition, a \ac{PWL} trajectory can be considered as an interval-based signal, which has a different property from an instance-based signal in that the time differences between each instance are not predefined. Obviously, with sufficient segments, a PWL trajectory can reconstruct the instance-based trajectory. 

% \begin{figure}
%     \centering
%     \includegraphics[width = 0.4\textwidth]{figs/dt_vs_pwl.png}
%     \caption{instance-based (left) and Interval-based (right) trajectory.}
%     \label{fig:dt_vs_ts}
% \end{figure}
\subsection{Qualitative STL Semantics for \ac{PWL} Trajectory}
Similar to the previous work \cite{Sun20223451}, we are only interested in specifications that indicate the robots to reach and avoid particular regions with the expected temporal behavior. Therefore, we use atomic predicates ${\lgPred}$ and its negation ${\tlNot\lgPred}$ to particularly indicate whether a \emph{linear waypoint segment} lies \emph{inside} or \emph{outside} a region $\mathcal{P}$. We assume that a region $\mathcal{P}$ can be approximated by convex polygon ${\polyAb = \{p \in \nSet{R}^d ~| Ap \leq h\}, A \in \nSet{R}^{r \times d}, h \in \nSet{R}^d}$. We investigate a 2D path-planning problem so $r = 2$. We show later in the experiments that the approximation assumption is not restrictive since it is sufficient to describe various reach-avoid specifications in path planning. 

Let the binary variable $z^\lgSpec_i$ indicate the statement ``segment $z_i$ (or \emph{any} signal instance in $[t_i, t_{i+1}]$) satisfies the formula $\lgSpec$", i.e., ${z^\lgSpec_i \lgEqual z_i \lgSatisfy \lgSpec}$ and 
${z^\lgSpec_i = \lgTrue \iff \sign(z^\lgSpec_i) = 1 \iff (\xi, t) \lgSatisfy \lgSpec, \forall t \in [t_i, t_{i+1}]}$.
With this notation, and w.l.o.g, let $\lgPred$ corresponds to region $\mathcal{P}$, i.e., $\lgPred$ holds true mean ``inside $\mathcal{P}$", and $\lgNeg\lgPred$ for ``outside $\mathcal{P}$". 
From here on, we have $\pi$ and $\lgNeg\pi$ are the atomic predicates that indicate 
${z_i^\lgPred \lgEqual Z_i(t) \in \mathcal{P}, \forall t \in [t_i, t_{i+1}]}$, and ${z_i^{\lgNeg\lgPred} \lgEqual Z_i(t) \not\in \mathcal{P}, \forall t \in [t_i, t_{i+1}]}$. We mathematically show in the following that these ``atomic predicates" are constructed from conjunctions and disjunctions of the aforementioned linear predicate introduced in Definition \ref{def:stl_syntax}
\begin{nalign} \label{eq:zpi_sdp}
     z_i^{{\lgPred}} \lgEqual &\bigwedge_{j = 1}^r \bigg( \frac{h^j - A^jp_i}{\norm{A^j}_2} \geq \epsilon  \lgAnd \frac{h^j - A^jp_{i+1}}{\norm{A^j}_2} \geq \epsilon \bigg), \\ 
     z_i^{\lgNeg {\lgPred}} \lgEqual & \bigvee_{j = 1}^r \bigg( \frac{A^j p_i - h^j}{\norm{A^j}_2} \geq \epsilon \lgAnd \frac{A^j p_{i+1} -  h^j}{\norm{A^j}_2} \geq \epsilon \bigg),
\end{nalign}
 % \begin{remark}
 % Whenever any segment $z_j$ is mentioned, the related waypoint's information is considered, i.e., ${z_j \hequal (p_j, t_j, p_{j+1}, t_{j+1})}$.    
 % \end{remark} 
% Briefly, \emph{Piecewise-Interval} trajectory considers the trajectory as connected piecewise linear segments (PWLs) that are represented by the waypoints. The authors in \cite{Sun20223451} proposed a sound qualitative encoding semantics for PWL w.r.t STL requirement.
%To encode the atomic predicates, i.e.,  and the negated one that reflects  $p$ 
where, $A^j, h^j$ are the coefficients of $j$-th rows of $A$ and $h$, i.e., one edge of the polygon. The positive space margin $\epsilon \in \nSet{R}$ is used to encounter the uncertain spatial deviation when robots track the segments. More importantly, each term of \eqref{eq:zpi_sdp} is \emph{linear} regarding $p_i$ or $p_{i+1}$ that obeys the assumption of using linear predicates. The following example explains the notation
 \begin{example} See Figure \ref{fig:convex_poly}. 
 Atomic predicates $\lgPred$ and $\lgNeg\lgPred$ corresponds to $\mathcal{P}$, i.e., 
 ${z_i \lgSatisfy \pi \iff Z_i(t) \in \mathcal{P}, \forall t \in [t_i, t_{i+1}]}$, ${z_i \lgSatisfy \neg\pi \iff Z_i(t) \not\in \mathcal{P}, \forall t \in [t_i, t_{i+1}]}$. We have $z_1 \not\lgSatisfy \pi$, ${z_1 \lgSatisfy \neg\pi}$, ${z_2 \lgSatisfy \pi}$, ${z_2 \not \lgSatisfy \neg \pi}$, ${z_3 \not\lgSatisfy \pi}$, ${z_3 \not\lgSatisfy \neg\pi}$, ${z_4 \not\lgSatisfy \pi}$, ${z_4\not\lgSatisfy \neg\pi}$.
% \begin{flalign*}
%     %z_i &\in \regPe \iff Z_i(t) \in \regPe, &&\forall t \in [t_i, t_{i+1}] \\ 
%     %z_i &\not\in \regPe \iff Z_i(t) \not\in \regPe, &&\forall t \in [t_i, t_{i+1}] \\        
%     %\pi &\lgEqual (z_i \in \regPe), &&\neg\pi \lgEqual (z_i \not \in \regPe)  \\
%     z_1 &\not\lgSatisfy \pi, &&z_1 \lgSatisfy \neg\pi \\
%      z_2 &\lgSatisfy \pi, &&z_2 \not \lgSatisfy \neg \pi \\
%      z_3 &\not\lgSatisfy \pi, &&z_3 \not\lgSatisfy \neg\pi \\
%      z_4 &\not\lgSatisfy \pi, &&z_4 \not\lgSatisfy \neg\pi &&&
%      \end{flalign*} 
 \end{example}  
 %For the "inside" predicate, if the starting and ending points of a segment are both in the same face of every edge, i.e., ${\forall j, b^j - A^jp - \epsilon \geq 0}$, we know that all points of this segment lie strictly inside the region with at least $\epsilon$ distance margin. Similarly, for the "outside" predicate, if there \emph{exists} an edge of the region such that both two starting and ending points lie outside, i.e., ${\exists j, A^jp - b^j - \epsilon \geq 0}$, then any point of this segment also lie outside of the region by at least $\epsilon$ distance margin \cite{Chuchu2020FGS}. 
%\thought{Note that by using this method, we approximate a region in practice by conjunction and disjunction of linear constraints. A smooth approximation method can be found in the work of \cite{Pang2017Smooth}. Besides, the $\epsilon$ distant margin is used to encounter the uncertainty of robots when they track the reference waypoints. By using an over spatial approximation, we can ensure that the robots always avoid the region as long as they maintain within the $\epsilon$ margin.}
% \begin{remark}  \label{rem:pwl_lost_negation}  
%     To be clear, the explicit definition of the above atomic predicates results in the loss in negation formula, i.e.,
%     \begin{nalign}
%       z_i^{{\lgPred}} \neq \lgNeg z_i^{{\lgNeg\lgPred}}  
%     \end{nalign}
%     It can be derived from \eqref{eq:sdp_pwl} and \eqref{eq:zpi_sdp} that we only have the following sufficient conditions ${z_i^{{\lgPred}} = \lgTrue \implies z_i^{{\tlNot\lgPred}} = \lgFalse}$ and $z_i^{{\tlNot\lgPred}} = \lgTrue \implies z_i^{{\lgPred}} = \lgFalse$. We \emph{do not} have ${z_i^{{\lgPred}} = \lgFalse \implies z_i^{{\tlNot\lgPred}} = \lgTrue}$ or ${z_i^{{\tlNot\lgPred}} = \lgFalse \implies z_i^{{\lgPred}} = \lgTrue}$. Such a situation occurs, for instance, when a segment intersects with a region. 
% \end{remark}
 For other operators, \cite{Sun20223451} proposed the qualitative semantics
\begin{nalign} \label{eqn:pwl_stl}
    z_{i}^{\stlAlways{a,b}\lgSpec} &\lgEqual \bigwedge_{j = 1}^{K} \left([t_j, t_{j+1}] \intersect [t_{i} + a, t_{i+1} + b] \neq \varnothing \implies z_j^\lgSpec \right) \\
    %
    z_{i}^{\stlEvtll{a,b}\lgSpec} &\lgEqual (t_{i+1} - t_i \leq b - a) \\ &\lgAnd  \bigvee_{j = 1}^{K} \left([t_j, t_{j+1}] \intersect [t_{i+1} + a, t_{i} + b] \neq \varnothing \lgAnd z_j^\lgSpec \right) \\
    %
    z_{i}^{\lgSpec_1\stlUntil{a,b}\lgSpec_2} &\lgEqual (t_{i+1} -t_i \leq b -a) \lgAnd \\ 
    &\bigvee_{j = 1}^{K} \bigg ([t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i +b] \neq \varnothing \lgAnd z_j^{\lgSpec_2} \\
    & \lgAnd \bigwedge_{l = 0}^j [t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \neq \varnothing \implies z_l^{\lgSpec_1} \bigg) 
    %
    % z_k^{\varphi_1 \stlUntil{a,b} \varphi_2} &= \lgAnd_{k = 0}^{H - 1} \left([t_j, t_{j+1}] \cup [t_i + a, t_{i+1} + b] \right) \\
\end{nalign}
\begin{figure} 
    \centering
    \includegraphics[width = 0.8\linewidth]{figs/poly.png}
    \caption{Examples of atomic predicates and its negation with \ac{PWL} segment. The grey area denotes the original polygon. The shrunk/bloated polygons by $\epsilon$ distant margin are the inner/outer dotted lines respectively.}  
    \label{fig:convex_poly}
\end{figure}
% \thought{notes: the until operator is derived from the following
% }
% \begin{align*}    z_{i}^{\lgSpec_1\stlUntil{a,b}\lgSpec_2} &: \exists t^\prime \in [t_{i+1} + a, t_i +b], \\
%     & \hspace*{-1cm} \bigvee_{j = 1}^{K} \left(t^\prime \in [t_j, t_{j+1}] \lgAnd z_j^{\lgSpec_2} \lgAnd \bigwedge_{l = 0}^j \left([t_l, t_{l+1}] \intersect [t_{i}, t_{i+1} +b] \implies z_l^{\lgSpec_1}\right)\right)
% \end{align*}
% \thought{Notes the strictness of the above encoding requiring $\lgSpec_1$ holds during the whole interval $[t_i, t_i+b]$
% }
%
% where $\mu(\xi(t)) \overset{\lgSpec}{\equiv} \mu(\xi(t^\prime))$ means that ${\mu(\xi(t)) \lgSatisfy \lgSpec \iff \mu(\xi(t^\prime)) \lgSatisfy \lgSpec}$.
%\end{definition}
%
% An equivalent representation of qualitative semantics is using the sign operator $\sign(.)$, i.e.,  
% \begin{nalign}
%     \sign(x): \nSet{R} \xrightarrow{} \{-1,0,1\} = 
%     \begin{cases}
%         1 & x \geq 0 \\
%         %0 & x = 0 \\
%         -1 & x < 0
%     \end{cases}, \\
%     \sign(x): \{0,1\} \xrightarrow{} \{-1,1\} = 
%     \begin{cases}
%         1 & x = 1 \\
%         -1 & x = 0
%     \end{cases}    
% \end{nalign}
% Let $z^\lgSpec_t$ indicate the qualitative value of a formula $\lgSpec$ and $(\xi, t)$, we have
% \begin{align*}
%     z^\lgSpec_t & \lgEqual (\xi, t) \lgSatisfy \lgSpec     
% \end{align*}
% From \eqref{eqn:qual_stl_semantics}, we define that ${(\xi, t) \lgSatisfy {\lgPred} \lgIff \mu^{\lgPred}(\xi(t)) \geq 0}$, this coressponds to
% \begin{nalign}
% z_t^{\lgPred} = \lgTrue &\iff \sign(z_t^{\lgPred}) =  \sign(\mu^{\lgPred}(\xi(t))) = 1 \\
% z_t^{\lgPred} = \lgFalse &\iff \sign(z_t^{\lgPred}) = \sign(\mu^{\lgPred}(\xi(t))) = -1 \\
% \end{nalign}

==> sections/review.tex <==
% \section{Literature Review} \label{sec:lr}
%Early usage of \ac{TL} as formal verification methods allows specifying and reasoning about the time-related behaviors of systems \cite{Baier2008}. %Researches in this area aim to construct rigorous syntax and semantics for reasoning and requirements formulation purposes, alos efficient implementation of algorithms of falsification and monitoring 
%Most of the applications are software falsification or verification, and monitoring, which are known as {model-checking} tool \cite{Clarke1986AutomaticVO, Emerson1996ModelCA, Manna1991TheTL, Alur1991TechniquesFA, Lamport1994TheTL, Alur2004ATL}. 
%Previous works by \cite{,,} provide a thorough overview of \ac{TL} and their variances, such as \ac{LTL}, \ac{MTL}, and \ac{STL}. {STL} offers a quantitative semantics for {continuous time} signal to evaluate signals over the reals \cite{Maler2004MonitoringTP}, thus is widely used in the context of control synthesis. 



==> sections/rewriting.tex <==
\section{Introduction \& Literature Review} 
Modern \ac{CPS} offers various potentials to revolutionize a wide range of applications, such as mobility-on-demand, coverage control, rescue operations, smart transportation, and precision agriculture \cite{AlZahrani2020UAVAP, Alotaibi2019LSARMC}. 
To formally handle the significant design challenges of the above safety-critical systems, it is essential to have an expressive and reliable mechanism that can capture the complexities.
\emph{Formal Methods} are powerful techniques that utilize logical and reasoning languages with rigorously defined syntax and semantics to support system developments, from requirements analysis to verification. Such methods allow us to express domain expertise unambiguously from natural languages. {One branch of Logic that has been extensively researched and widely used for formal verification is \ac{TL}, an expressive language capable of reasoning logical statements with respect to \emph{time} \cite{Baier2008}}. 
As an example, consider a path-planning problem that requires the robot to execute the following task, "\emph{eventually} visits region $A$ and stays there for $5$ time units". 
Such complex coupled spatial and temporal behaviors can be expressed with \ac{TL} formulas unambiguously. Moreover, from \ac{TL} specifications, it is possible to synthesize robots' trajectories that meet the expected spatial-temporal behaviors with automated algorithms, which is known as the \emph{formal synthesis} problem. Recent research focus on synthesis algorithms using \acrfull{STL}, a sub-branch of \ac{TL} supporting {continuous-time} signals over the reals and quantitative semantics  \cite{Maler2004MonitoringTP}, which allows evaluating the \emph{robustness}, i.e., \emph{degree of satisfaction}, of a signal regarding a specification. In other words, one may identify "How much" the system satisfies the requirement, which is essential for automated mission design and synthesis algorithms to encounter possible uncertainties in practice.  

\ac{STL} offers two quantitative semantics: \emph{space} and \emph{time} robustness. Space robustness indicates the spatial margin of a signal regarding specified thresholds, e.g., the \emph{safety-distance} between a trajectory and an obstacle. Formal \ac{STL} synthesis with space robustness is well-studied \cite{Raman2015ReactiveSF, Pang2017Smooth, Lindemann2019ControlBF}. 
One planning paradigm is using \emph{abstraction-based} method, e.g., \cite{Zhou_2015_OMP, Nikou_2016_CTP} transform a given \ac{STL} specification and the robot's dynamic into a product automaton to search for valid control sequences in the discrete space. A common bottleneck of these methods is that they rely heavily on the construction of the automata. Besides, these methods suffer from the problem of {state-space explosion}. Recent developments in automata theory offer modularized temporal testers \cite{ferrere2019real} aiming to make the abstraction-based methods more scalable \cite{Lindemann2020Eff}. 
%\thought{To our knowledge, none of these methods studied time-robustness.}
On the other hand, optimization-based approaches transform STL formulas into constraints related to the robot's trajectory. In this manner, a \ac{STL} control synthesis problem can be formulated into an \ac{MPC}/ optimization problem which then be solved by available commercial solvers. \cite{Karaman2008OptimalCO, Raman2015ReactiveSF} proposed the encoding rules to transform \ac{STL} with linear predicates into linear constraints with mixed binary and continuous variables, then the obtained model is solved with \ac{MILP}. The authors in \cite{Pang2017Smooth} proposed an approximation method to avoid the computational burden of binary variables in
\ac{MILP}, which enables the problem to be solved with Sequential Quadratic Programming.
%The constraints are simultaneously solved
%with mixed continuous and binary variables.  
%Many works aim to decompose \ac{STL} formulas into short-horizon formulas to achieve more efficient optimization problems,  \cite{Fiaz_2020_FCR, Leahy2022FDTLS}.
%For space robustness, \cite{Pang2017Smooth} proposed approximation methods to synthesize trajectory with Sequential Quadratic Programming. 
\cite{Leung2020BackpropagationTS} introduced methods to compute the gradient of the \ac{STL} robustness and allow synthesis with gradient-descent optimization. 
Although optimization-based approaches are straightforward, {they do not scale well due to the complexity of the constructed \ac{MILP}. In particular, from an \ac{STL} formula, the generated constraints are imposed on \emph{each} discretized trajectory instances, which implies that the \ac{MILP} increases in the number of binary and continuous variables proportionally with the planning time horizon.
%consists of a high number of mixed binary and continuous variables \cite{Lindemann2019ControlBF, zhang2023modularized}}. 
%Besides, they suffer from the scalability issue due to the fact that solving \ac{MILP} is \emph{hard} in general. 
{Some studies try to achieve an efficient synthesis. \cite{Lindemann2019ControlBF} suggest constructing time-varying \ac{CBF} from a fragment of \ac{STL} that renders the forward invariant set that satisfies the formula. This approach offers scalability but further attention is required for the general construction of \ac{CBF} functions for various complex specifications. The work \cite{zhang2023modularized} studies a decomposition method to transform long STL formulas into combinations of modularized ones, thus reducing the computational time of \ac{MILP}. }

Compared to space robustness, less attention was put on \emph{time robustness}. The work \cite{Donze2010RSTL} first defined time-robustness for STL formulas. Afterward, \cite{akazaki2015time, Rodionova2022TRTL} further investigated in the context of monitoring and control synthesis. With time robustness, we can evaluate the performance quantitatively regarding time, e.g., "the requirement is satisfied with \emph{large time-margin}, or just \emph{in-time}." Such a property is essential as it is hard in practice to assign fixed-time missions, or robots always encounter ubiquitous delays, early starts, or reactive disturbances in the environment. The authors in \cite{Rodionova2022TRTL} proposed a novel strategy to encode time robustness into linear constraints for discretized signal, which allows time-robust synthesis with \ac{MILP}. This approach also suffers from the aforementioned scalability issue.

{Informally, efficient synthesis from \ac{STL} formula is an open problem. We are motivated to investigate a scalable synthesis method that also offers time-robustness. Our method is directly inspired by the work  \cite{Chuchu2020FGS, Sun20223451} which proposed a novel hierarchical path-planning method using \ac{PWL} signal and their \emph{qualitative} semantics for formal synthesis. 
%a high-level planner to generate \ac{PWL} signal and a low-level tracking controller. 
\ac{PWL} signal considers a trajectory as a sequence of 
waypoints consisting of timestamps and values.  
}
In fact, \cite{Chuchu2020FGS, Sun20223451} shows that various planning problems can be represented by a much less number of waypoints compared to the number of dense-discretized trajectory instances, especially for long-time-horizon planning problems. In this manner, the size of the constructed \ac{MILP} does not scale proportionally with the time horizon but depends solely only on the available number of waypoints. None of these previous works considered time-robustness. We, therefore, propose and investigate the concept of time-robustness for \ac{PWL} signal. The contribution of our study is summarized below
% Our method is strongly related to the previous works by \cite{Chuchu2020FGS, Sun20223451}. The authors in \cite{Chuchu2020FGS} introduce path planning methods using PWL path, which considers a trajectory as sequences of time-stamp waypoints. In this manner, we don't have to impose the constraints on the system at each time-step. Besides, many tasks in practice can be represented through a reasonable \ac{PWL} segment, thus enabling an optimization problem with fewer constraints. \cite{Sun20223451} proposes a qualitative semantics for \ac{PWL} signal to synthesize the desired waypoints.
%Our methods do not impose constraints on each discretized state at each time step of the system as used in \cite{Rodionova2022TRTL}, but instead just introduce constraints on the less number of \ac{PWL} segments that can describe various tasks in practice. \thought{Can you pls help me think of some way to clarify instance-based and interval-based here directly.}

\noindent \textbf{Contributions.} 
\begin{itemize} [leftmargin = *]
    \item \emph{Definition and Quantitative Semantics of Time-Robustness for PWL Signal}: 
    %We formulate the time-robustness STL semantics for \ac{PWL} signal. 
    The notion of time-robust STL was introduced in \cite{Donze2010RSTL} and formally studied in \cite{Rodionova2022TRTL} for instance-based signal. Different from previous works, we study and propose the time-robust quantitative STL semantics for \ac{PWL} signal. We first formally defined time robustness for \ac{PWL} signal, then mathematically propose and scrutinize the soundness of the quantitative time-interval semantics.
    
    \item \emph{Time-Robust STL Path Planning:} We formulate a novel hierarchical time-robust formal synthesis problem using \ac{PWL} Signal.
    \item \emph{MILP Encoding}: We propose an encoding strategy to transform the studied semantics into a \ac{MILP} problem.
    \item \emph{Experiments}: the synthesis algorithm implemented on MATLAB and numerical experiments to verify the soundness and our complexity analysis.
\end{itemize}
\textbf{Organization} 
%Section \ref{sec:lr} provides a review of literature studying space-time robust path planning from \ac{STL} formulas. 
Section \ref{sec:prel} introduces the preliminaries including the mathematical notations, qualitative semantics of \ac{STL}, and \ac{PWL} signal. Section \ref{sec:mr} presents the definition and quantitative semantics of time-robust \ac{STL} with \ac{PWL} signal. Section \ref{sec:pf} formally formulates the synthesis problem and introduces a hierarchical planning framework. Section \ref{sec:milp_enc} proposes an encoding strategy to construct a \ac{MILP} for the proposed semantics. Section \ref{sec:bm} provides the numerical experiments result to evaluate the soundness and the performance of our approach. Section \ref{sec:concl} concludes our study.

==> sections/rw_VB.tex <==
\subsection{{Time Robustness} Encoding for \ac{PWL} signal}
\begin{itemize} [leftmargin=*]
 \item Atomic predicates $\pi / \neg \pi$ indicate whether \emph{a segment} lies inside / outside $\mathcal{P}$. They are constructed from the conjunction and disjunction of linear predicates according to \eqref{eq:zpi_sdp}. We apply the above encoding to obtain the \emph{linear constraints} for two binary variables $z_i^\lgPred$ and $z_i^{\neg\lgPred}$.  
 %With these constraints, these two binary variables $z_i^\lgPred$ and $z_i^{\neg\lgPred}$ that indicate whether segment $z_i$ satisfy/violate the atomic predicate $\lgPred$ or $\neg\lgPred$.
In the following, we use the right-time robustness $\rtrobzj{i}^{{\lgPred}}$ to explain the encoding. A similar strategy can be applied for the left time robustness. Let $\rtrobzj{i}^{{\lgPred}}$ be the right {\tr} of segment $z_i$ regarding $\lgPred$, we show how we can generate linear constraints such that $\rtrobzj{i}^{{\lgPred}}$ correspond to the definition of {\tr} in \eqref{eq:pwl_prop_tr_strict}. To this end, we adapt the ``counting" encoding concept proposed by the authors in \cite{Rodionova2022TRTL} as follows.
%Recall the definition of $\rtrobzj{i}^{{\lgPred}}$ from \eqref{eq:pwl_prop_tr_strict}.
% Recall the definition of $\rtrobzj{i}^{{\lgPred}}$ as
% \hspace*{-0.75cm}\begin{nalign} \label{eq:ss}
%     \rtrobzj{i}^{{\lgPred}} &= \sign(z_i^{\lgPred}) \sum_{j = i+1}^{i + k}(t_{j+1} - t_j), \\ 
%     k &= \defkpeq \\
%     %
%     %\max_{\{0, 1, 2,\cdots, K\}} s.t. ~\forall i^\prime \in \{i+1, \cdots, i+k\}, \sign(z_i^{\lgPred}) = \sign(z^{\lgPred}_{i^\prime})\\
%     \rtrobzj{i}^{{\lgPred}} &= 0 \text{ if } k = 0.
% \end{nalign}
% Intuitively, if $z_i^{\lgPred} = \lgTrue$, we "aggregate" the time interval of the successive segment as long as these segments hold true regarding ${{\lgPred}}$. If the immediate successive segment doesn't hold, i.e., $z_{i+1}{\lgPred} = \lgFalse$, $z_i$ has $0$ right-{\tr}. Same explanation is applied for $z_i^{\lgPred} = \lgFalse$, but we have to multiply $-1$ additionally due to the sign operator $\sign(z_i^{\lgPred})$.
% In particular, they proposed the counting variables $c^1_i$ and $c^0_i$:  
% \begin{align} \label{eq:counting_milp}
%     c^1_i &= (c^1_{i+1} + 1)z_i, \\
%     c^0_i &= (c^0_{i+1} + 1)(1 - z_i).
% \end{align}
%
% We introduce the right-time robustness encoding for PWL segments wrt a proposition ${\lgPred}$ in the following. For any linear segment with timestamps $t_i, t_{i+1}$ and the symbolic binary variable $z_i$ determines the correctness of this segment wrt a proposition ${\lgPred}$, 
We first define the \emph{time-aggregating} variables $\Delta t^1_i$ and $\Delta t^0_i$ as follows
\begin{nalign} \label{eq:t_aggre}
    \Delta t^1_i &= (\Delta t^1_{i+1} + \delta t_i)z_i^{\lgPred},
    \Delta t^0_i = (\Delta t^0_{i+1} - \delta t_i)(1 - z_i^{\lgPred}),
\end{nalign}
with ${\delta t_i = t_{i+1} - t_i}$, ${\Delta t^1_{K-1} = \Delta t^0_{K-1} = 0}$. In the above formula, $\Delta t^1_i$
% From definition \ref{def:time_rob}, time robustness is defined as the strict time margin of the successive segments (not considering the interval of the current segment), we subtract this time amount from the variables defined in \eqref{eq:t_aggre}, i.e., 
% \begin{align*}
%     \Delta t^1_i &= \delta t^1_{i} - z_i\delta t_i \\
%     \Delta t^0_i &= \delta t^0_{i} + (1 - z_i)\delta t_i.
% \end{align*}
aggregates the time interval of the successive segments $z_{i+1}$ if $z^\lgPred_{i+1} = z^\lgPred_{i} = 1$, while  $\Delta t^0_i$ aggregate the negative time interval, i.e.,  $-\delta t_i$ if $z^\lgPred_{i+1} = z^\lgPred_{i} = 0$. Moreover, since \eqref{eq:t_aggre} is recursive, the aggregation continues until $z_{i+1} \neq z_{i}$. This corresponds to the $\sum$ operator used in \eqref{eq:pwl_prop_tr_strict}. 
In fact, the purpose of using two variables $\Delta t^1_i$ and $\Delta t^0_i$ is to distinguish the sign operator $\sign(z_i^\lgPred)$ defined in \eqref{eq:pwl_prop_tr_strict}. Since these variables are disjunctive, i.e., ${\Delta t^1_i \neq 0 \implies \Delta t^0_i = 0}$ and vice versa \cite{Rodionova2022TRTL}, they can be combined into $\Delta t^1_i  + \Delta t^0_i$. We have the time robustness of one segment below 
% \begin{align}
%     \Tilde{\theta}^{{\lgPred}}_{+,i} = \Delta t^1_i  + \Delta t^0_i.
% \end{align}
\begin{subequations} 
\begin{align} 
   \rtrobzj{i}^{{\lgPred}} &= \Delta t^1_i  + \Delta t^0_i + \left(- z_i^{\lgPred}\delta_i + (1 - z_i^{\lgPred})\delta_i \right) \label{eq:tr_raw}\\ 
    &= z_i^{\lgPred}\Delta t^1_{i+1} + (1 - z_i^{\lgPred})\Delta t^0_{i+1} \label{eq:right_time_rob}.
\end{align}
\end{subequations}
The last summand in \eqref{eq:tr_raw} is explained by the fact that the {\tr} defined in \eqref{eq:pwl_prop_tr_strict} does not contain the time interval $\delta_i$ of the current segment $z_i$.
% Finally, the time robustness is obtained by subtracting (or adding) the time interval of the current segments depending on $z_i^{\lgPred})$, i.e.,
% \begin{align} \label{eq:right_time_rob}
%     {\theta}^{{\lgPred}}_{+,i} &= \Tilde{\theta}^{{\lgPred}}_{+,i} - z_i^{\lgPred}\delta_i + (1 - z_i^{\lgPred})\delta_i \\ 
%     &= z_i^{\lgPred}\Delta t^1_{i+1} + (1 - z_i^{\lgPred})\Delta t^0_{i+1}
% \end{align}
To summarize, the time robustness $\rtrobzj{i}^{{\lgPred}}$ is encoded by introducing additional aggregating variables for each segment, then imposing linear constraints for the recursive formulas in \eqref{eq:t_aggre}, and also leverage \eqref{eq:multi_xb} to impose linear constraints that reflect the multiplication of binary and continuous variables in \eqref{eq:right_time_rob}.  
%To express ${\theta}^{{\lgPred}}_{+,i}$ with linear constraints, the primary challenge is to encode \eqref{eq:t_aggre}, i.e., the multiplication of a continuous and a binary variable by using \eqref{eq:multi_xb}. 
% The primary encoding challenge for ${\lgPred}$ is to express $\eqref{eq:t_aggre}$ as linear constraints. This can be realized through the encoding strategy for the product of a continuous and binary variable $y = xb$, i.e., ${-Mb \leq y \leq Mb,~ x - M(1 - b) \leq y \leq x + M(1 - b)}$, with positive $M$ as the sufficient large upper bound of $x$.

% \begin{remark}
% Different from the discrete-time semantics, we don't subtract the time-interval of the current segment as shown in \cite{RodionovaTRTL} because $\delta t_i$ is already strict positive and considered as the time robustness of the segment $i$. 
% \end{remark}
% %
% \thought{
% \begin{remark}
% The time robustness is "counted" in   \cite{RodionovaTRTL} as can be seen in \eqref{eq:counting_milp}. In our "aggregating" encoding \eqref{eq:right_time_rob}, it is computed from the continuous time variables $t_i$. This may explain why DT could find a solution faster.
% \end{remark}
% }
\item For temporal operators, we instruct the encoding for the ``eventually" ($\tlEvtll$), the other operators can be done similarly. Recall the expression from \eqref{eq:evtll_time_rob_strict}, let $\trob^*$ be $\trobzj{i}^{\stlEvtll{a,b}\lgSpec}$, we introduce $K-1$ additional binary variables $[b_1 \cdots b_{K-1}]$ and impose the following constraints
\begin{subequations} 
\begin{flalign}
%& b_{ij}^\intersect \lgEqual [t_j, t_{j+1}] \intersect [t_{i+1} +a, t_i + b] \neq \varnothing, t_{i+1} - t_i \leq b - a, \label{eq:timeintrs_evtll_tr}\\
& b_{ij}^\intersect \lgEqual (t_{i}+b - t_j \geq \epsilon_t) \lgAnd (t_{j+1} - (t_{i+1} +a) \geq \epsilon_t) \notag \\
& ~~~~~~ \lgAnd \left(t_{i+1} - t_i \leq b - a\right), \forall j \in \{1 \cdots K\}; \label{eq:timeintrs_evtll_tr}\\
& \trobzj{j}^\lgSpec - (1- b_{ij}^\intersect)M \leq \trob^*, \forall j \in \{1 \cdots K\}; \label{eq:geq_evtll_tr} \\
& \trob^* \leq \trobzj{j}^\lgSpec + (1- b_{j})M, \forall j \in \{1 \cdots K\}; \label{eq:evtll_tr_leq}\\  
& b_{ij}^\intersect \geq b_j, \forall j \in \{1 \cdots K\}; \sum_{j = 1}^K b_j = 1. \label{eq:supremum_exists}
\end{flalign}
\end{subequations} 
First, in \eqref{eq:timeintrs_evtll_tr}, the binary variable $b^\intersect_{ij}$ with $\epsilon_t \in \nSet{R}_{\geq 0}$ indicates whether two time-intervals $[t_j, t_{j+1}]$ and ${[t_{i+1} +a, t_{i} +b]}$ intersects.
%[t_{i1}, t_{i2}]$ and $[t_{i+1} +a, t_i + b]$ intersect through the constraints ${b^\intersect_{ij} \lgEqual (t_{j2} - t_{i1} \geq \epsilon_t) \lgAnd (t_{i2} - t_{j1} \geq \epsilon_t) }$,  
If $b^\intersect_{ij} = \lgTrue$, they intersect, else they don't.
Equation \eqref{eq:geq_evtll_tr} implies that $\trob^*$ is greater or equal to the time robustness of \emph{any} segments that intersect with $[t_{i+1} +a, t_i + b]$. Meanwhile, \eqref{eq:evtll_tr_leq} guarantees that $\trob^*$ is bounded by $\trobzj{j}^\lgSpec$ whenever $b_{j} = 1$. Finally, \eqref{eq:supremum_exists} ensures that the supremum belongs to the given set that intersects, i.e, $b_j = 1 \implies b_{ij}^\intersect = 1$. Besides, $\sum_{j = 1}^K b_j = 1$ ensures that the supremum exists.
\end{itemize}

